Nonlinear Initialization Methods for Low-Rank Neural Networks

We propose a novel low-rank initialization framework for training low-rank deep neural networks -- networks where the weight parameters are re-parameterized by products of two low-rank matrices. The most successful prior existing approach, spectral initialization, draws a sample from the initialization distribution for the full-rank setting and then optimally approximates the full-rank initialization parameters in the Frobenius norm with a pair of low-rank initialization matrices via singular value decomposition. Our method is inspired by the insight that approximating the function corresponding to each layer is more important than approximating the parameter values. We provably demonstrate that there is a significant gap between these two approaches for ReLU networks, particularly as the desired rank of the approximating weights decreases, or as the dimension of the inputs to the layer increases (the latter point holds when the network width is super-linear in dimension). Along the way, we provide the first provably efficient algorithm for solving the ReLU low-rank approximation problem for fixed parameter rank $r$ -- previously, it was unknown that the problem was computationally tractable to solve even for rank $1$. We also provide a practical algorithm to solve this problem which is no more expensive than the existing spectral initialization approach, and validate our theory by training ResNet and EfficientNet models (He et al., 2016; Tan & Le, 2019) on ImageNet (Russakovsky et al., 2015).

==> old_learning_theory.tex <==

\section{Theory for Learning Low-Rank Networks} \label{sec:theory_learning}

% TODO: refer to the exact lemma/corollary / theorem numbers in the references for the theorems we copy paste

% TODO: move some of this around (we mention it after the problem statement, we probably mention some of it in related work)
In this section we consider the problem of learning optimal low-rank approximations to fully-connected, shallow neural networks. We study this problem in a simple setting to gain insight into methods for learning low-rank deep networks in general, and because it is an interesting open learning theory problem. It is of particular interest since in the literature, the only computationally tractable cases for learning even ReLU activations require the realizable assumption, even under the assumption of Gaussian marginals. All positive results for computationally tractable learning up to (non-approximate) additive error require making this assumption, and various hardness results (for instance, statistical queries (SQ) lower bounds \citep{feldman2016statistical}) are known for a variety of agnostic settings. In our case, since we wish to learn a low-rank approximation, we are automatically not in the realizable setting: however, we know a lot more structure about the responses than in the arbitrary agnostic setting, and we also do not have to deal with noise, so it is plausible that our learning problem is tractable.  

\subsection{Problem Statement and Assumptions}

% TODO: in anticipation of a potential misunderstanding: we should make a remark that our results don't contradict anything about the problem of learning a ReLU activation being non-convex.
% indeed, our algorithm requires non-convex optimization results:
% 1) actually recovering the m ReLUs is non-trivial to prove (existing work does this in the realizable setting).
% 2) solving "kernel PCA" on the weight matrix W is also non-convex.
% PCA itself is not a convex problem (we are maximizing a _convex_ function! not minimizing it). 

% TODO: define a "problem" environment and fix references so that they call it "Problem x" rather than "problem solved in Definition x"
% todo: rename so population is R and empirical is R_hat
\begin{problem}[Shallow Low-Rank Learning Problem]\label{prob:learning_prob_statement}
Consider the objective
\begin{align}
    \mathcal{R}(Y) 
    := \mathbb{E}_{x \sim \mathcal{N}(0, I)}\left[\left\|\sigma_{\txt{ReLU}}(x^\top Y) - \sigma_{\txt{ReLU}}(x^\top W)\right\|_2^2\right] \label{eq:population_objective}
\end{align}
\vspace{-4ex}

where $\sigma_{\txt{ReLU}}(x) = \max(0, x)$ is the ReLU activation, $W, Y \in \mathbb{R}^{d \times m}$, and $W$ are fixed ground-truth full-rank weights.
Let $\txt{opt} := \mathcal{R}\left(Y^*\right)$, where $Y^*$ is the argmin over matrices of rank $r$.
If a learner is only given samples $\left\{\left(x, \sigma_{\txt{ReLU}}(x^\top W)\right)\right\}_{x \sim \mathcal{N}(0, I)}$, what are the computational and sample complexities of finding the optimal rank $r$ matrix $\hat{Y}$, such that with probability at least $1 - \delta$,
$
\mathcal{R}(\hat{Y})  < \txt{opt} + \epsilon
$?
\end{problem}

See Remarks~\ref{rem:factorizing_Y} and \ref{rem:conv_arch} to see how the statement applies to factorized and convolutional models.

There are several interesting features of this problem with respect to the problems studied in the existing literature.


Many papers have studied related problems in a variety of settings \citep{goel2016reliably, goel2019time, soltanolkotabi2017learning, chen2021learning, diakonikolas2020approximation, goel2020statistical, goel2020superpolynomial}.
Compared to previous work, the setting we study is a) not realizable but, b) there is significant structure on the outputs, and there is no noise. We assume Gaussian marginals similar to previous work. 
See Section~\ref{sec:related_work} and also Ch. $3$ of \citet{chen2021rethinking} for a thorough discussion of recent related work in statistics and deep learning theory.

It is thus currently open whether there exists an algorithm that runs in polynomial time and sample complexity to solve this problem; it is also open whether we can solve this using a gradient (or any SQ) method, as existing lower bounds do not directly rule out such an algorithm for this setting.

We prove that for the shallow low-rank learning problem with the ReLU activation, there is a computationally efficient SQ algorithm. The full proofs are in Section~\ref{subsec:sec2_proofs} of the Appendix. In the following sections we briefly sketch the key features of the arguments.

\subsection{The Algorithm}

First we present an efficient algorithmic framework called \algB (NKP) for computing the optimal low-rank matrix given knowledge of the full-rank weights for a broad family of nonlinearities. Using \algname for ReLU, we give the first efficient learning algorithm for the shallow low-rank ReLU learning problem. A few definitions will be useful first.


\begin{definition}[Nonlinearity Kernel]\label{def:nonlinearity_kernel}
Given a univariate activation function $\sigma$, define the associated \textbf{nonlinearity kernel}\footnote{In prior literature, this function is highly related to the C-Map concept derived and applied in \citet{saxe2014exact, poole2016exponential, martens2021rapid}, and is identical up to normalization. It is worth noting that the setting in which these works derive the C-Map is considerably different from ours: normality arises due to taking infinite-width limits of deep networks and assumptions on weight initialization distributions, rather than an assumption on the input data distribution.} by:
$
k_{\sigma}(x, y) := \E{z \sim \mathcal{N}(0, 1)}{\langle \sigma(x^\top z), \sigma(y^\top z)\rangle}
$.
\end{definition}

Note this is a positive semi-definite kernel \citep{scholkopf2002learning, martens2021rapid}.

\begin{lemma}[Feature Map for Nonlinearity Kernels]
Given the Hermite coefficients \citep{ODonnell14} for a nonlinearity $\sigma$, it is easy to construct the feature map $\phi: \mathbb{R}^d \to \mathcal{L}_2\left(\mathcal{N}(0, I)\right)$ such that
$
k_{\sigma}(x, y) = \langle \phi(x), \phi(y) \rangle
$.
See Section~\ref{subsec:hermite} for more details.
\end{lemma}
We also define a family of activation functions which satisfy an inversion condition on $\phi$ , which is necessary for \algname to work.
\begin{definition}[Family of Easily Invertible Activation Functions]\label{def:easily_invertible}
We define a family of \textbf{easily invertible activations} $\mathcal{A}$ as:
$
\mathcal{A} := \left\{\sigma: \mathbb{R} \to \mathbb{R}: \E{z \sim N(0, 1)}{z \sigma(z)} > 0\right\}
$.
\end{definition}
See Remark~\ref{rem:invertible_activation_examples} for examples (e.g., ReLU, Swish).
Now we present the \algname algorithm:
\vspace{-1.5ex}
\begin{algorithm}
\caption{\algname (NKP) Algorithm}\label{alg:mixnmatch}
\begin{algorithmic}[1]
\REQUIRE $W \in \mathbb{R}^{d \times m}$, (optional) $K \in \R^{m \times m}$, rank $r < d < m$, easily invertible activation function $\sigma$
\STATE Compute kernel $K = k_{\sigma}(W, W)$ if not given.
\STATE Compute $V\Lambda V^{\top} = \txt{SVD}\left(K, r\right)$. \quad \slash\slash~rank-$r$ SVD
\STATE \textbf{Return:} $Y^* = W V V^{\top} \in \R^{d \times m}$. 
\end{algorithmic}
\end{algorithm}
Our shallow low-rank ReLU learning algorithm consists of recovering $W$ approximately from samples using gradient descent (which is efficient in the realizable setting \citep{soltanolkotabi2017learning}), recovering the kernel matrix $K_{\sigma}$ approximately from samples with an empirical estimate, and then applying \algnameshort with the ReLU activation.


\begin{algorithm}
\caption{Shallow Low-Rank ReLU Learning}\label{alg:lowrank_shallow_learning}
\begin{algorithmic}[1]
\REQUIRE Sample access to $\left\{\left(x, \sigma_{\txt{ReLU}}(x^{\top}W)\right)\right\}_{x \sim \mathcal{N}(0, I)}$ for unknown $W \in \mathbb{R}^{d \times m}$, $r < d < m$
\STATE Use gradient descent to recover $\hat{W}$ up to Frobenius error $\epsilon_W$ with probability $\geq 1 - \delta_W$ by learning the ReLU for all $m$ columns using $n_W(\epsilon_W, \delta_W)$ samples. % note: can separately recover the kernel without using GD
\STATE Compute  $\hat{K} = \frac{1}{N}\sum_{i = 1}^N \sigma(x_i^{\top}W)\sigma(x_i^{\top}W)^{\top}$ up to Frobenius error $\epsilon_K$ with probability $\ge 1 - \delta_K$ using $N = n_K(\epsilon_K, \delta_K)$ samples.
\STATE \textbf{Return:} $\hat{Y} = \NKP\left(\hat{W}, \hat{K}, r, \sigma_{\txt{ReLU}}\right)$. 
\end{algorithmic}
\end{algorithm}


\subsection{Analysis}

Now we prove our main theorem: Algorithm~\ref{alg:lowrank_shallow_learning} efficiently solves Problem~\ref{prob:learning_prob_statement}.

\begin{theorem}[Shallow Low-Rank ReLU Learning is Computationally and Statistically Efficient]\label{thm:efficient_learning}
Consider Problem~\ref{prob:learning_prob_statement}, where $W \in \R^{d \times m}$ is the matrix of full-rank parameters defining the one-hidden-layer ReLU function.
Algorithm~\ref{alg:lowrank_shallow_learning} is an efficient learning algorithm for recovering the optimal low-rank matrix up to additive generalization error $\eps$ with probability at least $1 - \delta$. Both the sample complexity and computational complexity of learning rank-$r$ ReLU approximation are $\poly\left(R, d, m, \frac{1}{\eps}, \log\left(\frac{1}{\delta}\right), \|W\|_2, \frac{1}{\lambda_r - \lambda_{r - 1}}, r\right)$, where $R$ is a bound on the $\ell_2$ norms of the columns of $W$, $\|W\|_2$ is the spectral norm of $W$, and $\lambda_r, \lambda_{r -1}$  are the $r^{th}$ and $(r - 1)^{st}$ eigenvalues of $K_{\txt{ReLU}}$ respectively.
\end{theorem}
\vspace{-15pt}
\begin{proof}
[Proof Sketch]

To prove this theorem, we put together 1) a computationally and statistically efficient method for estimating the kernel matrix up to additive Frobenius error (Theorem~\ref{thm:relu_kernel_learning}); 2) a computationally and statistically efficient method for estimating $W$ up to additive Frobenius error (Corollary~\ref{cor:learning_W}); 3) a computationally efficient algorithm for recovering the best low-rank approximation $Y^*$ given knowledge of $W$ and the kernel matrix $K_{\txt{ReLU}}$ (\algnameshort Algorithm, Theorem~\ref{thm:proof_alg1}); 4) perturbation bounds on the eigenvectors of an approximate kernel matrix combined with perturbation bounds on approximate $W$ to get a perturbation estimate of the final $Y^*$ (Lemma~\ref{lem:perturbation_bound1}). Putting all these elements together yields the result. 
Please refer to the full proof in Section~\ref{subsec:sec2_proofs} in the Appendix.
\end{proof}
\vspace{-2ex}
We remark in Remarks~\ref{rem:spectral_properties_bounds} that if we assume an average case setting over $W$, we can make use of random matrix theory to replace the eigenvalue gap and spectral norm terms as well as improve the degrees in the bounds in Theorem~\ref{thm:efficient_learning}. In Remark~\ref{rem:improving_degrees}, we mention some other avenues for improving the degrees in the bounds.

Given Theorem~\ref{thm:efficient_learning}, we broadly note where the difficulties in Problem~\ref{prob:learning_prob_statement} lie:

\begin{corollary}[Reduction to Realizable Learning and Kernel Learning] \label{cor:reduction}
Learning shallow, low-rank, easily invertible activation functions over Gaussian data up to additive error is computationally efficient given an efficient learning algorithm for noiseless realizable activation learning over Gaussian data and an efficient algorithm for learning the nonlinearity kernel matrix given i.i.d. samples.
% todo: how efficient does the learning algorithm have to be (use the estimates for how precisely you need to learn W_hat -- we don't need to get into this.
\end{corollary}


Now we proceed to provide the key non-trivial theorems required for the proof of Theorem~\ref{thm:efficient_learning}.
First we prove the correctness of \algnameshort for \textit{any} activation function satisfying the easily invertible condition (Definition~\ref{def:easily_invertible}), though it is likely possible to extend beyond this condition (see Remark~\ref{rem:easy_invertibility_not_necessary}).


\begin{theorem}[Correctness \& Efficiency of NKP]\label{thm:proof_alg1}
The \algnameshort algorithm optimizes the population objective of Problem~\ref{prob:learning_prob_statement} for any easily invertible activation function, given $W \in R^{d \times m}$ and target rank-$r$, in $\mathcal{O}\left(m^3 + m^2\cdot (r + d)\right)$ time.
\end{theorem}
\vspace{-15pt}
\begin{proof}
[Proof Sketch]

The key idea is to apply kernel PCA to the full-rank parameter matrix $W \in \R^{d \times m}$, noting that $W$ is not a data matrix. Then, we need to invert the feature map of the nonlinearity kernel in order to recover the best low-rank parameter matrix $Y \in \R^{d \times m}$ (we are left with a matrix in $\R^{r \times m}$ after kernel PCA). This step is possible if the kernel is easily invertible (Definition~\ref{def:easily_invertible}).
See the full proof in Section~\ref{subsec:sec2_proofs} in the Appendix.
\end{proof}





We also require the following non-trivial result on the sample complexity of learning the ReLU nonlinearity kernel (it is necessary to learn the kernel separately, see Remark~\ref{rem:why_learn_kernel_separately}):

\begin{theorem}[ReLU Kernel Learning Sample Complexity]\label{thm:relu_kernel_learning}
Let
$
\hat{K}_{\sigma} = \frac{1}{N}\sum_{k = 1}^N \sigma(x_k^{\top}W)\sigma(x_k^{\top}W)^{\top}
$,
where the columns of $W \in \R^{d \times m}$ satisfy $\|W_i\|_2 \leq R$ for $i \in [m]$, $\sigma(a) = \max(0, a)$ for $a \in \R$ is the ReLU activation function and where we draw $N$ samples from the data distribution $\left\{\left(x_k, \sigma(x_k^{\top}W)\right)\right\}_{k = 1}^N$ with $x_k \sim \mathcal{N}\left(0, I_{d \times d}\right)$ i.i.d. for all $k \in [N]$. Now suppose 
$
N \geq \Omega\left(R^4\cdot d^2 \cdot m^2\cdot\frac{1}{\eps^2}\cdot \min\left(d\log^2\left(\frac{1}{\delta}\right), \frac{1}{\delta}\right)\right),
$
then with probability $\ge 1 - \delta$, we have $\|\hat{K}_{\sigma} - K_{\sigma}\|_F \leq \eps$.
\end{theorem}
\vspace{-15pt}
\begin{proof}
[Proof Sketch]
We proceed by analyzing the concentration of the individual kernel values, followed by a union bound over a discretization of the compact space of possible $W$ (Lemma~\ref{lem:eps_net_union_bound}). 
This analysis is very similar to the analysis in \citet{rahimi2007random}; however, we must make use of a more involved argument involving the dependent Hanson-Wright inequality (Lemma~\ref{lem:hanson_wright_dependent}). The key challenge is that our kernel estimate is not a bounded or Lipschitz function in the random samples and has complicated dependencies. The full proof is in Section~\ref{subsec:sec2_proofs} in the Appendix.
\end{proof}


% TODO: do these todos go in appendix or main paper?

% TODO: make note that the eigenvalue gap in the Davis-Kahan is unavoidable in general

% TODO: make note that we can always try to choose ranks so that we avoid this eigenvalue gap (since the actual eigenvectors themselves are not determinable within an eigenspace (though, we don't know W in advance)

% TODO: if W is drawn from a gaussian (or other distributions), work characterizing the eigengap distribution exists and we can bound it with a constant. similarly for maximal eigenvalue (Marchenko Pastur, Wigner Semi-Circle, Tracy-Widom) stuff is relevant - what assumptions should we remark on?



%% TODO: REMARK ON lambda_r - lambda_{r - 1} and \|W\|_2 for assumptions on W coming from standardized Gaussian etc!
%% these quantities are bounded (cite Tao & Vu paper for instance? others?) so that they're basically a constant in the case of Gaussian W. Good to mention this so that it's clear that the result is efficient for Gaussian W (average case setting). with high probability.









%TODO: mention non-homogenity of our problem setting. i think it is fine for one-hidden-layer networks.



%%%%%%%%%%%%%%%%%%%%%%%% OLD STUFF to draw from %%%%%%%%%%%%%%%%%%%%%

% Motivation for studying this setting: 

% we use gradient method , ideally would show that gradient method can solve.
% however, we can give an SQ algorithm, so hardness results likely don't apply. 
% we study noiseless setting (w/fixed W) since this is relevant to our init alg
% in more complicated settings, we may not be able to simply just give an SVD alg for solving (e.g. if there are weird things like batch norm, conv layers, etc)
% so, we want to justify approach which only gets sample access to sigma(Wx) -- e.g. a learning problem. -- this is more general / applies to potentially harder versions of the distillation problem, where we distill different chunks of network at a time possibly.
% so we study a simple setting there are show it's possible with a non-SQ gradient alg. Also fills a gap in the literature. the fact that it's noiseless but not-realizable is also interesting.
% would ideally show that we can use a gradient method to implement hte SQ algorithm as well, to complete the story.



%We can specialize this and first ask whether it is possible to efficiently learn a rank$-1$ network. 
%We will also assume that the nonlinearity is a ReLU for simplicity.

% note: pay attention to rotational invariance and so on.

%Let 
%\[
%f^*(x) = \sigma\left(Wx\right)
%\]
%where $\sigma(z) = \max(0, z)$ is the ReLU nonlinearity, , $W \in \mathbb{R}^{m \times d}$ are the parameters of the network, and $x \in \mathbb{R}^d$. 

%Then we wish to solve the following learning problem: Consider the hypothesis class $\mathcal{F} = \left\{g_{U, V}(x) = \sigma(UV^\top x): U \in \mathbb{R}^{m \times k}, V \in \mathbb{R}^{d \times k}\right\}$. Then we wish to find
%\[
%U^*, V^* = \textnormal{arg}\min_{U, V} \mathbb{E}_{x \sim N(0, I_d)}\left[\left\|g_{U, V}(x) - f^*(x)\right\|_2^2\right]
%\]

%Furthermore we want to ask how tractable this problem on average over draws of $W$'s entries from i.i.d. Gaussians. 
%In particular, we would like to know if this problem is tractable to solve with gradient methods. 




% wrong, we don't need to do this
%We make some progress on this problem by demonstrating that if we take the limit as the width goes to infinity, while maintaining a fixed rank scale, it is possible to solve the distillation problem for Gaussian weights and Gaussian marginals efficiently. The proof idea is essentially that in this limit, we attain the realizable setting, and thus ideas from \citep{soltanolkotabi2017learning} can be applied to our problem.

%\begin{theorem}
%Suppose the rank scale of the network is $\gamma$, the width of the network is $m$, and the input dimension is $d$.
%Then we consider a low-rank parameterization $U, V$ such that $U \in \mathbb{R}^{m \times \gamma*m}, V \in \mathbb{R}^{d \times \gamma*m}$.
%Suppose $m \to \infty$. % need to make this more precise.
%Then, finding $\hat{U}, \hat{V}$ such that
%\[
%\mathbb{E}_{x \sim N(0, I_d)}\left[\left\|g_{\hat{U}, \hat{V}}(x) - f^*(x)\right\|_2^2\right] < \textnormal{opt} + \epsilon
%\]
%with at least constant probability is possible in time polynomial in $d, m, 1/\epsilon$.
%\end{theorem}
%\begin{proof}
%[Proof Sketch]

%\end{proof}





%(See the related work).

%\cite{soltanolkotabi2017learning} % learning via gradient descent
% - learns ReLU with square loss (with any regularizer)
% - assumes labels are generated by ground-truth model (corresponding to fixed weight vector)
% - Gaussian marginals
% - shows that gradient descent init at 0 converges to optimum at linear rate. 
% method: 
% doesn't directly apply to our setting




%\cite{chen2021learning} % deep nets
% - learn deep ReLU network with depth > 2
% - Gaussian inputs
% - algorithm is polynomial in dimension but exponential in other quantities including "rank" k
% - weights of deep net have rank k
% - output is 1 neuron
% - exact outputs given by true network (no noise)
% - square loss
% - method: filtered PCA + net arguments
% - they note: all existing algorithm results for Gaussian inputs hold only for depth 2 networks and make at least one of two assumptions: a) weight matrix is full rank/ well-conditioned; b) vector at output has all positive entries
% (most are the first assumption, only DKKZ20 "Algorithms and sq lower bounds for PAC Learning 1 hidden lyear ReLU networks" has the second assumption; it turns out not to be necessary.
%\cite{chen2020learning} % polynomials is related ideas but in a different setting
% can be directly applied to our problem to get poly(d) sample/computational complexity, but exponential in 1/eps^2 for error epsilon in both sample and computational complexity. 

%\cite{chen2021efficiently} % query learning
% query learning setting, not directly relevant except as another possible extension
% we could consider a query learning setting for initialization rather than arbitrary sampling
% since we have black box access to the model
% could attempt to extend their results in the low-rank direction
% - learns 1-hidden-layer ReLu network with respect to Gaussian inputs given query access
% - poly(d, 1/eps, log(1/delta)) query complexity
% - can we give a query based alg for recovering low-rank model?
% - they look at learning worst-case networks from queries
% - not directly applicable to our setting

%\cite{dudeja2018learning} % connection to multi-index models
% different setting, mention in passing

%\cite{goel2019time} 
% 

%\cite{goel2020superpolynomial}

%\cite{goel2020statistical}
% setting: H is a function class on R^n, D is a distribution on R^n x R s.t. marginal on R is standard Gaussian. 
% labels don't necessarily come from some other kind of ReLU (e.g. no full rank vs. low rank here), they can be completely worst case, and we want to compare to the best opt. additionally we don't even have that if there were a function, it would be drawn from a Gaussian weights distribution. (the distribution on labels can be whatever the heck one wants it to be). 
% prove: statistical query lower bounds (rule out GD). exponential in dimension statistical queries needed. 
% focus is on ReLU regression as usual (lower bound). even in Gaussian marginals setting; but our setting is plausibly easier.
% method: reduction. result of DKKZ20 and GGJ+20 for SQ lower bounds on agnostically depth-two neural nets (activation applied to sum of nonlinearities); they show that individual nonlinear activation function regressions can be used (in an SQ way) to solve the original problem (requires looking at surrogate loss and functional gradient descent via Frank-Wolfe and ensuring the steps are SQ-implementable). 
% given our setting, I think an efficient SQ algorithm isn't be ruled out (have to double check the DKKZ20 and GGJ+20 SQ lower bounds; i bet they make use of properties of function family that may not hold when functions are drawn from Gaussians and there actually is a "full rank" ground truth rather than arbitrary label distribution). 

%\cite{diakonikolas2020approximation}

%\cite{daniely2020hardness} % hardness of PAC learning with natural weights
% computational notion of hardness: RSAT (refuting random K-SAT formulas)
% setting: randomly choose a depth-2 random network which outputs a single neuron, where second layer weights are all 1.
% then efficient learning means: for a random weight matrix, and every data distribution D (that may depend on W), given noiseless sample access, algorithm runs in polytime and success w/at least constant probability over choice of W such that
% generalization error is smaller than a constant.
% this problem is RSAT-hard for natural choices of weight distributions like Gaussians.






% refer to Surbhi's work, Sitan's work, and possibly the multi-index model literature.

%Sample and Computational Complexity

% The below points should come up in the analysis of the above:
% Simply, they are:
% 1. Bias of the Gspectral learning problem (it's not agnostic)
% 1.5 Bias of the distribution matching problem
% 1.6. How bias of distribution matching problem changes with width


==> old_related_work.tex <==
\section{Appendix: Additional Related Work}\label{sec:related_work}

%% THIS IS ALL USEFUL FOR FOLLOWUP PAPER ON LEARNING THEORY PROBLEM!!!
Here we fill in some of the related work not previously described in the paper.
%\textbf{Orthogonal Initialization}
%Our successful approach uses approximately orthogonal initialization. Many other works study the benefits of orthogonal initialization. One set of works empirically studies impact on optimization convergence, especially in large deep networks via the formalism of dynamical isometry (pennington, etc papers on dynamical isometry, recent edge of chaos paper, mean field theory). One theoretical work examines optimization in the deep linear setting, and demonstrate that orthogonal initializations exponentially speeds up the convergence of gradient descent in that setting. Another set of work argues for the benefits of using orthogonal matrices for kernel approximations of attention matrices (choromanski + his other works on orthogonal init being better). 

\textbf{Single-Index Models}

% mention related work on kernel approximation? not critical... nice to have?
% similarly, people have studied concentration for lipschitz kernels -- so that's a class of kernels for which results exist, but they don't necessarily correspond to activation function kernels (https://arxiv.org/pdf/1909.03347.pdf) 
% seems like most of it applies to rahimi-recht style random features, and they can make Lipschitz assumption.
% we can't make lipschitz assumption, which is why our stuff requires novel analysis
% cite the papers that are related (Danica Sutherland 1506.02785, perhaps choromanski http://proceedings.mlr.press/v84/choromanski18a/choromanski18a.pdf ? first gives better concentration that doesn't apply to our setting; second isn't that related since they are talking about choosing different r.f. maps basically which concentrate better, orthogonal to our question.
% might be the case that we are the first to give a concentration bound like this for estimating the kernel (for unknown W) -- if so, mention this somewhere? "to the best of our knowledge..."
% note that our setting is: given sample data of a type we can't choose (in the learning theory problem statement), estimate the kernel.
% emphasize that focus in literature seems to be on shift-invariant kernels, and they all can use lipschitz assumption
% also emphasize that our setting is different: we have _unknown INPUTS to the kernel (columns of W) (which are restricted to some family of possible W), and we are trying to estimate the kernel values of those unknown inputs from samples. this is a different setting from the literature as far as I can tell, so this is a novel problem requiring a novel solution.
% so indeed the problem is different from:
% 1) random features regression (Song Mei et al 2021) + many more
% 2) learning the best kernel (Sinha-Duchi 2016) 
% we genuinely care about uniform convergence to the kernel approximation as its own end goal, since we want to use the eigendecomposition of that kernel, and the literature doesn't seem to have studied the uniform convergence of kernels beyond shift-invariant kernels which have lipschitz or bounded properties. thus this is a novel result in that line of work as well.

Results for efficiently learning realizable activations directly provides one of the ingredients for efficient learning results like Theorem~\ref{thm:efficient_learning} (see Corollary~\ref{cor:reduction}), so we might wonder for what activations other than ReLU it is possible to efficiently solve the problem.

The general problem of learning an activation is known as learning a single-index model in the statistics community (see \citet{dudeja2018learning} for a comprehensive review of this body of work). 

Many existing works have studied the problem of properly learning various activations in the realizable setting \citep{klivans2004learning, kalai2009isotron, kakade2011efficient, ge2018learning, zhong2017recovery, janzamin2015generalization, dudeja2018learning}, and if those activations also satisfy our easily invertible condition, we can efficiently learn a low-rank approximation for these activations as well (simply replacing gradient descent with whatever the efficient realizable learning algorithm is). 

Notably, the conditions often require monotonicity and Lipschitz assumptions, smoothness assumptions, Fourier-theoretic low-degree polynomial approximation assumptions, or are for specific activations, most commonly the ReLU, sigmoid, and tanh activations. The GLMtron algorithm of \citet{kakade2011efficient} and the tensor-recovery initialized gradient methods of \citet{zhong2017recovery} in particular apply to broad classes of activation functions.

Most of the methods for learning non-linear activations do not apply to learning the swish, which is non-monotonic and non-symmetric about the origin. Since swish is smooth, however, we can adapt methods from the literature on single-index models to learn a single Swish function. In particular, the single-index algorithm of \citet{dudeja2018learning} applies to our setting which has a $\poly(N, d)$ runtime, where $N$ is the number of samples, though the sample complexity is $\mathcal{O}(1/\epsilon^2)$ and $\poly(d)$.

The square activation corresponds to the extremely well-studied phase retrieval problem. Our \algname algorithm does not apply (the square activation is even), but existing work has studied low-rank phase retrieval in different settings \citep{vaswani2017low, nayer2020provable}. 

\textbf{Computational Learning Theory for Neural Networks}

Several works \citep{goel2019time, goel2020statistical, goel2020superpolynomial, soltanolkotabi2017learning, goel2016reliably} derive the computational and statistical hardness of learning a single ReLU function $\sigma(w^{\top}x)$ in various settings. Such works typically assume the data distribution is marginally Gaussian on the examples, and focus on definitions of generalization error with respect to square loss. There is a significant difference in attainable results in the agnostic learning setting compared to the realizable setting. In the realizable setting, where the noiseless labels come from a planted model $\sigma({w^*}^Tx)$, the results are positive: \citep{soltanolkotabi2017learning} proved that projected gradient descent, initialized at $0$, converges at a linear rate (in square loss) to the planted $w^*$ with optimal sample complexity. 

However, in various other settings, hardness results exist. In the agnostic learning setting with Gaussian marginals, \citep{goel2020statistical} demonstrates that any statistical-query (SQ) based algorithm --- which includes most known learning algorithms including stochastic gradient descent --- requires exponential in dimension many statistical queries to learn a ReLU up to additive error $1/10$ with respect to the squared loss. 

On the other hand, \citep{goel2019time} gives an efficient approximation algorithm with runtime $\textnormal{poly}(d, 1/\epsilon)$ for finding the best fitting ReLU in an agnostic learning setting which achieves error $\mathcal{O}\left(\textnormal{opt}^{2/3}\right) + \epsilon$, where $\textnormal{opt}$ is the square loss of the best fitting ReLU, when the marginal distribution of the features is log-concave. \citep{diakonikolas2020approximation} significantly improves this result by providing an algorithm which has runtime $\textnormal{poly}(d, 1/\epsilon)$ which, under the assumption of marginal log-concavity (and no assumptions on the noise/response), is able to recover a vector $w$ such that the corresponding ReLU function has square loss at most $\mathcal{O}(\textnormal{opt}) + \epsilon$. Note that \citep{goel2019time} proved that achieving $\textnormal{opt} + \epsilon$ is computationally hard (via reduction to learning sparse parities with noise), so this is essentially the best result we can hope for. Also some assumption on the marginal distribution of the features is necessary, otherwise the problem is NP-hard \citep{diakonikolas2020approximation}.

% the approx algorithm SQ. is it gradient / nicely implementable? GLMtron? it is - they do projected gradient on a surrogate objective. in particular can check Section 4 of Surbhi's general SQ paper to see that they use same surrogate loss as the approximation paper for the functional gradient boosting reduction. so SQ ruled out for additive approx, but not O(opt) + additive approx. how bad is constant in the O? and how does it translate to our setting? constant may not be too bad, but still desirable to remove it.

% AN INTERESTING QUESTION FOR US: SGD vs Adam on our objective. what about a mirror descent w.r.t. low rank spectahedron style regularizer to learn just rank 1 weights? Is that tractable? / provably efficient? Also, how can we use diakonikolas results for our rank 1 setting directly? Do we lose something in doing so? double check this. how about how good is SGD specifically? we want to get at low rank structure here.

In the average case PAC learning setting, \cite{daniely2020hardness} showed that learning a randomly initialized two-layer network with a single output neuron in square loss reduces to refuting random $k$-SAT formulas, a computational hardness assumption known as RSAT, for various natural choices of initialization distributions. This paper shows that it is often average-case computationally hard to learn a randomly initialized two-layer network over arbitrary data distributions.

Thus, taken separately, both the Gaussian marginals assumption and the average case weights assumption can still lead to hardness for additive approximation in square loss for various simple neural networks, though we can evade such issues if we are willing to give up a constant factor in the optimal error. It is quite reasonable to hope to avoid such constant factors from a practical standpoint, and the existing computational hardness results do not apply to our setting.

In our setting, we consider both these assumptions simultaneously, and while our hypothesis class does not contain the ground-truth function (and thus we are not in the realizable setting), the ground-truth function is also not arbitrary: It is a full-rank variant of our function, and our setting is noiseless. Furthermore, we are in the setting where the output of our function is not $1$-dimensional -- none of the existing papers study this case. Furthermore, the distribution of the vector outputs is not arbitrary as is the case in the agnostic PAC setting considered in many papers that consider learnability with respect to Gaussian marginals: We assume that the output is a specific function drawn from a class of specific distributions (but our hypothesis class simply does not contain this function) -- we can hope to exploit this extra information about the problem setting to evade existing hardness results. Thus, the existing lower bounds on SQ algorithms (like SGD) do not apply to our setting given the assumptions we make.


% their algorithm is not CSQ (correlational statistical queries). 
There is also recent work \citep{chen2020learning} considering the problem of learning low-rank deep networks with respect to Gaussian marginals in the realizable setting; but to the best of our knowledge there are no such other works. They are able to give an algorithm whose running time is polynomial in the dimension (and an exponentially large function in the network's other parameters as well as in $1/\epsilon$, where $\epsilon$ is the additive square loss generalization error). Their work does not directly apply to our setting since they are in the realizable setting (we want to learn the best low-rank approximation to the full rank network).



==> old_section2_proofs.tex <==
\subsection{Proofs for Section~\ref{sec:theory_learning}} \label{subsec:sec2_proofs}

%%% SOME LEMMAS ARE RIGHT (KERNEL APPROX + PERTURBATION, BUT MAIN THM IS WRONG!!!
%%% TODO(knv): adapt into something else different paper?
First we prove the correctness of \algnameshort.

%% THIS THEOREM IS WRONG!!!!
%% --> can't assume phi(Y*) is low rank!!!
\begin{theorem}[Correctness and Efficiency of \algname]
The \algname algorithm optimizes the population objective defined in Problem~\ref{prob:learning_prob_statement} for any easily invertible activation function, given $W \in R^{d \times m}$ and target rank $r$, in time $\mathcal{O}\left(m^3 + m^2\cdot (r + d)\right)$.
\end{theorem}
\begin{proof}
We have
\begin{align}
\begin{split}
 &\mathbb{E}_{x \sim \mathcal{N}(0, I)}\left[\left\|\sigma(x^{\top}Y) - \sigma(x^{\top}W)\right\|_2^2\right] 
 \\
 &= k_{\sigma}\left(Y, Y\right) + k_{\sigma}\left(W, W\right) - 2k_{\sigma}\left(Y ,W\right) 
 \\
 &= \left\|\phi(Y) - \phi(W)\right\|_2^2  
\end{split}
\end{align}
where $\phi$ is the feature map defining $k_{\sigma}(x, y)$, applied column-wise to $Y, W$. Then, we can perform the standard manipulations to recover the kernel SVD objective, by writing $\phi(Y) = UU^{\top}\phi(W)$ for some orthogonal rank $r$ $U$: 
\begin{align}
\begin{split}
    &\argmin_{Y} \|\phi(Y)\|_2^2 - 2\txt{Tr}\left(\phi(Y)^{\top}\phi(W)\right)
    \\
    &= \argmax_{U^{\top}U = I_{r \times r}} 2\txt{Tr}\left((I - UU^{\top})\phi(W)\phi(W)^\top(I - UU^{\top})\right) 
    \\
    &- \left\|(I - UU^{\top})\phi(W)\right\|_F^2 
    \\
    &= \argmax_{U^{\top}U = I_{r \times r}} \txt{Tr}\left(U^{\top}\phi(W)\phi(W)^{\top}U\right)
\end{split}
\end{align}
Now we can write the kernel form of the optimization problem to get the dependence on $K = \phi(W)^{\top}\phi(W) \in \R^{m \times m}$, which we also note is a positive semi-definite symmetric matrix. We now reproduce the standard ideas of \citet{scholkopf1998nonlinear, scholkopf2002learning}. 
Note we can write $U = \phi(W)A$ for $A \in \R^{m \times r}$, since we have $\phi(W)\phi(W)^\top U = U\Sigma$ and thus $U = \phi(W)\left(\phi(W)^{\top}U\Sigma^{-1}\right)$.
Let $Z = U^{\top}\phi(W) = A^{\top}\phi(W)^{\top}\phi(W) = A^{\top}K_{\sigma}$. Finally, noting that our current objective is maximizing $\txt{Tr}\left(ZZ^{\top}\right)$, we write 
\begin{align}
\begin{split}
    ZZ^{\top} &= U^{\top}\phi(W)\phi(W)^{\top}U = A^{\top}K_{\phi}^2A
\end{split}
\end{align}
and thus we get 
\[
\argmax_{A^{\top}K_{\phi}A = I_{r \times r}} \txt{Tr}\left(A^{\top}K_{\phi}^2A\right)
\]
Writing $B = \sqrt{K_{\phi}}A$, we get
\[
\argmax_{B^{\top}B = I_{r \times r}} \txt{Tr}\left(B^{\top}K_{\phi}B\right)
\]
Then $B^* = V \in \R^{m \times r}$, where $V$ corresponds to the top $r$ eigenvectors of $K_{\phi}$. We can then write $Z^* = {A^*}^{\top}K_{\phi} = V^{\top}\sqrt{K_{\phi}} = V^{\top}V\Sigma V^{\top} = \Sigma V^{\top} \in \R^{r \times m}$, the resultant optimal low-dim projection.

However, we want to actually recover $Y^*$. Thus, we write in the expanded feature space
\begin{align}
\begin{split}
\phi(Y^*) &= U\Sigma V^\top
\\
Y^* &= \phi^{-1}\left(U\Sigma V^\top\right)
\end{split}
\end{align}
We have written $\phi^{-1}$ to refer to a column-wise inverse transformation -- in order for this step to be valid, such a column-wise inverse has to exist. In our case, this is guaranteed by the fact that the activation is easily invertible (Definition~\ref{def:easily_invertible}). Since the Hermite coefficient $c_1 := \E{z \sim N(0, 1)}{z \sigma(z)}$ is positive by easy invertibility, for some column vector $x \in R^{d}$, the associated feature map $\phi(x)$ has $d$ rows which correspond to $c_1 * x$. We only need to identify those rows and divide by $c_1$ to recover $x$; thus the operation $\phi^{-1}$ is well-defined (even if the feature-map is a mapping to Hilbert space!). However, we want to avoid computing $U$, the corresponding top eigenvectors of $\phi(W)\phi(W)^{\top}$ which lie in the feature map space, since this can be expensive (or impossible in the case of Hilbert space feature maps). Again easy invertibility saves us: We only care about the relevant $d$ rows of the feature map corresponding to the entries of $Y^*$. Thus, we have
\[
Y^* = \frac{1}{c_1}\overline{U} \Sigma V^{\top}
\]
where $\overline{U} \in \R^{d \times r}$ is the low-rank approximation of $U$ localized to the correct $d$ rows. However, we still need to calculate $\overline{U}$. Notice that considering the full-rank case, we get
\begin{align}
\begin{split}
    W &= \phi^{-1}\left(U_{\txt{dim}(\phi) \times m}\Sigma_{m \times m} V_{m \times m}^{\top}\right)
    \\
    &= \frac{1}{c_1}\overline{U}_{d \times m}\Sigma_{m \times m} V_{m \times m}^{\top}
\end{split}
\end{align}

We emphasize here that this expression is \textit{not} the standard singular value decomposition of $W$ -- in particular, $\overline{U}$ does not have orthogonal columns, and $\Sigma, V$ are already defined by the kernel SVD. However, we then get the following expression:
\[
\overline{U}_{d \times m} = c_1\cdot WV_{m \times m}\Sigma_{m \times m}^{-1}
\]
To get the corresponding low-rank approximation $\overline{U}$, we simply choose the top singular values according to $\Sigma$ and their corresponding singular vectors in $V$:
\[
\overline{U} = c_1\cdot WV_{m \times r}\Sigma_{r \times r}^{-1}
\]
Tnen, we can plug this expression back into $Y^*$:
\[
Y^* = \frac{1}{c_1}\overline{U} \Sigma V^{\top} = W V V^{\top}
\]
where $V$ is the top $r$ eigenvectors of $K_{\phi}$, thus proving the result.

Since the algorithm only requires taking the SVD of the $m \times m$ kernel matrix and some matrix multiplications, the algorithm is $\poly(d, m)$ time. 
\end{proof}

\begin{remark}[Easy Invertibility Is Possibly Not Necessary] \label{rem:easy_invertibility_not_necessary}
Here, we have made the easily invertible assumption which is necessary for the \algname framework to work, namely that we can efficiently recover $x$ given $\phi(x)$. However, it is plausible that a variant of \algnameshort works for other activation functions, namely modifying the recovery step. One can write down a set of nonlinear equations in $x$ based on the non-zero coefficients of $\phi$ to recover the input (the number of coefficients you need and the nonlinearities involved impact the feasibility and efficiency of \algnameshort).
\end{remark}

Now we prove that Algorithm~\ref{alg:lowrank_shallow_learning} efficiently solves the shallow low-rank ReLU learning problem.


% THEOREM IS WRONG DUE TO ABOVE BEING WRONG (but the sub-parts are correct). 
\begin{theorem}[Shallow Low-Rank ReLU Learning is Computationally and Statistically Efficient]
Consider Problem~\ref{prob:learning_prob_statement}, where $W \in \R^{d \times m}$ is the matrix of full-rank parameters defining the one-hidden-layer ReLU function.
Algorithm~\ref{alg:lowrank_shallow_learning} is an efficient learning algorithm for recovering the optimal low rank matrix up to additive generalization error $\eps$ with probability at least $1 - \delta$. Both the sample complexity and computational complexity of learning rank-$r$ ReLU approximation are $\poly\left(R, d, m, \frac{1}{\eps}, \log\left(\frac{1}{\delta}\right), \|W\|_2, \frac{1}{\lambda_r - \lambda_{r - 1}}, r\right)$, where $R$ is a bound on the $\ell_2$ norms of the columns of $W$, $\|W\|_2$ is the spectral norm of $W$, and $\lambda_r, \lambda_{r -1}$  are the $r^{th}$ and $(r - 1)^{st}$ eigenvalues of $K_{\txt{ReLU}}$.
\end{theorem}
\begin{proof}
To prove this theorem, we put together 1. a computationally and statistically efficient method for estimating the kernel matrix up to additive Frobenius error; 2. a computationally and statistically efficient method for estimating $W$ up to additive Frobenius error; 3. a computationally efficient algorithm for recovering the best low-rank approximation $Y^*$ given knowledge of $W$ and the kernel matrix $K_{\txt{ReLU}}$; 4. perturbation bounds on the eigenvectors of an approximate kernel matrix combined with perturbation bounds on approximate $W$ to get a perturbation estimate of the final $Y^*$. Putting all these elements together yields the result. 

First we define 
\[
\eps_K := \left\|K_{\txt{ReLU}} - \hat{K}_{\txt{ReLU}}\right\|_F
\]
and 
\[
\eps_W := \|W - \hat{W}\|_F
\]
We now list the various results we need:
\begin{enumerate}
    \item Theorem~\ref{thm:relu_kernel_learning} gives an algorithm which requires $N = \mathcal{O}\left(\frac{R^4\cdot d^2 \cdot m^2}{\eps_K^2}\cdot \min\left(d\log^2\left(\frac{1}{\delta_K}\right), \frac{1}{\delta_K}\right)\right)$ samples and runtime $\mathcal{O}\left(N\cdot d \cdot m\right)$ to learn the kernel $K_{\sigma}$ up to additive Frobenius error $\eps_K$ with probability at least $1 - \delta_K$.
    \item Corollary~\ref{cor:learning_W} due to \citet{soltanolkotabi2017learning} gives an algorithm which requires $N = \mathcal{O}\left(d + \log(m/\delta_W)\right)$ samples and runtime $\mathcal{O}\left(N\cdot d\cdot m\cdot \log\left(\frac{R\cdot \sqrt{m}}{\eps_W}\right)\right)$ to learn the matrix $W$ up to additive Frobenius error $\eps_W$ with probability at least $1 - \delta_W$.
    \item Algorithm~\ref{alg:mixnmatch} finds the optimal rank $r$ $Y^*$ given exact $W$ and $K_{\txt{ReLU}}$ in time $\mathcal{O}\left(m^3 + m^2\cdot (r + d)\right)$ (though see \citet{allen2016lazysvd} for faster methods than $\mathcal{O}(m^3)$ for SVD depending on other parameters of the matrix). 
    \item Algorithm~\ref{alg:lowrank_shallow_learning} uses Algorithm~\ref{alg:mixnmatch} as a subroutine applied to estimates of the kernel matrix $\hat{K}_{\txt{ReLU}}$ and the parameter matrix $\hat{W}$, which have time and sample complexities given directly above.
    \item Lemma~\ref{lem:perturbation_bound1} bounds the gap in population error between the optimal rank-$r$ matrix $Y^*$ and the estimated matrix $\hat{Y}$ which is the output of Algorithm~\ref{alg:lowrank_shallow_learning} in terms of the Frobenius norms of the additive approximation errors of the estimates of $\hat{K}_{\txt{ReLU}}$ and $\hat{W}$ used by Algorithm~\ref{alg:lowrank_shallow_learning}:  
\end{enumerate}
\begin{align}
\begin{split}
    \mathcal{R}(\hat{Y}) - \mathcal{R}(Y^*) &\leq 8R^2 \cdot m \cdot \sqrt{\eps_K\cdot \frac{\|W\|_2}{\lambda_r - \lambda_{r - 1}} + \eps_W}
\end{split}
\end{align}


%In order to get this result, we need several bounds. First, we need generalization error bounds for estimating $W$ via gradient descent and for estimating $K_{\phi}$ from samples. Then, we need to bound the additive generalization error for our main objective defined in Problem~\ref{prob:learning_prob_statement} in terms of the approximations due to using samples. 
All that remains is to plug in the error estimates and take union bounds across the kernel learning subroutine and the $W$-learning subroutine to get the overall additive generalization error bound. First we set
\[
\eps = 8R^2 \cdot m \cdot \sqrt{\eps_K\cdot \frac{\|W\|_2}{\lambda_r - \lambda_{r - 1}} + \eps_W}
\]
Let $\eps_W = \frac{1}{2}\gamma^2$ and $\eps_K = \frac{1}{2}\gamma^2\cdot \frac{\lambda_r - \lambda_{r - 1}}{\|W\|_2}$. Then, $\eps = 8R^2\cdot m \cdot \gamma$ and we choose 
\[
\eps_W = \frac{1}{2}\left(\frac{\eps}{8R^2\cdot m}\right)^2
\]
and
\[
\eps_K = \frac{1}{2}\left(\frac{\eps}{8R^2\cdot m}\right)^2\cdot \frac{\lambda_r - \lambda_{r - 1}}{\|W\|_2}
\]
to give us total generalization error $\eps$.

Now we take union bounds across kernel learning and $W$-learning and simply set probability of failure for kernel learning and the probability of failure for $W$-learning to both equal $\delta/2$ -- this step just adds a constant factor to the bound and does not affect the asymptotic complexity. So, the total sample complexity across both kernel and $W$-learning is dominated by the kernel learning sample complexity and is thus overall bounded by
\[
N = \mathcal{O}\left(\frac{R^{12}\cdot d^2 \cdot m^6 \cdot \|W\|_2^2}{\eps^4 \cdot \left(\lambda_r - \lambda_{r - 1}\right)^2}\cdot \min\left(d\log^2\left(\frac{1}{\delta}\right), \frac{1}{\delta}\right)\right)
\]
The overall time complexity is bounded by 
\[
\mathcal{O}\left(N\cdot d\cdot m\cdot \log\left(\frac{R^5\cdot m^{2.5}}{\eps^2}\right) + m^3 + m^2\cdot (r + d) \right)
\]

Thus, both the time complexity and the sample complexity are $\poly\left(R, d, m, \frac{1}{\eps}, \log\left(\frac{1}{\delta}\right), \|W\|_2, \frac{1}{\lambda_r - \lambda_{r - 1}}, r\right)$.

\end{proof}


Now we proceed with the development of the required lemmas to prove Theorem~\ref{thm:efficient_learning}.
First we restate the main theorem of \citet{soltanolkotabi2017learning} for reference:

\begin{lemma}[Learning Realizable ReLU with Gradient Descent \citep{soltanolkotabi2017learning}] \label{thm:soltanolkotabi17}
Consider the setting of learning a single ReLU $\max(0, {w^*}^{\top}x)$ from noiseless samples (e.g., one column of $W$, so $w^* \in \R^d$) over standard Gaussian marginals. Assume $\|w^*\|_2 \leq R$. Then if we run projected gradient descent initialized from $0$ over a batch of size $n$, where $n \geq d$, with probability at least $1 - 9\exp\left(-\Theta(n)\right)$, we have that the gradient descent updates $w_t$ satisfy
\[
\left\|w_t - w^*\right\|_2 \leq 2^{-t} \cdot R
\]
Or, defining $\eps = \left\|w_t - w^*\right\|_2$, 
\[
t \geq \log\left(\frac{R}{\eps}\right)
\]
giving the required number of iterations of gradient descent to reach $\ell_2$ error $\eps$ for learning $w^*$, thus giving a total computational complexity $\poly\left(n, d, \log\left(R/\eps\right)\right)$.
\end{lemma}

\begin{corollary}[Learning $W$ from Samples] \label{cor:learning_W}
We can run gradient descent $m$ times -- once for each column of $W$ -- so the guarantee holds simultaneously
over all $m$ learning problems. So the probability of failure is set to be $\delta$, we choose
$n = \Theta\left(d + \log\left(\frac{m}{\delta}\right)\right)$ (via union bound). Then, to ensure that 
$\|W^* - \hat{W}\|_F \leq \eps$, we choose $t = \log\left(\frac{R\cdot \sqrt{m}}{\eps}\right)$ and run that many steps for each of the $m$ columns of $W$. Thus, the sample complexity is $n = \poly\left(d, \log(m), \log(1/\delta)\right)$ and the computational complexity is $\poly\left(m, d, n, \log\left(R / \eps\right)\right)$.
\end{corollary}

We will make use of a dependent random variables version of the Hanson-Wright inequality for quadratic forms, which yields sub-exponential tails:

\begin{lemma}[Dependent Hanson-Wright over Sub-Gaussians \citep{zajkowski2020bounds}]\label{lem:hanson_wright_dependent}
Suppose $x \in R^d$ is a sub-gaussian random variable satisfying $\E{x}{\exp(t\cdot x)} \leq \exp\left(K^2 t^2 / 2\right)$ for all $t \in \R$. Then for matrix $A \in \R^{d \times d}$, we have
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|x^{\top}Ax - \E{x}{x^{\top}Ax}\right| \geq t\right) 
    \\
    &\leq 2\exp\left(-\min\left\{\frac{t^2}{16 C^2 K^4\|A\|_{\txt{nuclear}}^2}, \frac{t}{4CK^2\|A\|_{\txt{nuclear}}}\right\}\right)
\end{split}
\end{align}
where $C$ is a universal constant and $\|\cdot\|_{\txt{nuclear}}$ refers to the nuclear norm defined by the absolute sum of the singular values of the matrix.
\end{lemma}

Now we prove a learning result for the kernel matrix.

% TODO: mention related work on kernel approximation
% seems like most of it applies to rahimi-recht style random features, and they can make Lipschitz assumption.
% we can't make lipschitz assumption, which is why our stuff requires novel analysis
% cite the papers that are related (Danica Sutherland 1506.02785, perhaps choromanski http://proceedings.mlr.press/v84/choromanski18a/choromanski18a.pdf ? first gives better concentration that doesn't apply to our setting; second isn't that related since they are talking about choosing different r.f. maps basically which concentrate better, orthogonal to our question.
% might be the case that we are the first to give a concentration bound like this for estimating the kernel (for unknown W) -- if so, mention this somewhere? "to the best of our knowledge..."
% note that our setting is: given sample data of a type we can't choose (in the learning theory problem statement), estimate the kernel.
% emphasize that focus in literature seems to be on shift-invariant kernels, and they all can use lipschitz assumption
% also emphasize that our setting is different: we have _unknown INPUTS to the kernel (columns of W) (which are restricted to some family of possible W), and we are trying to estimate the kernel values of those unknown inputs from samples. this is a different setting from the literature as far as I can tell, so this is a novel problem requiring a novel solution.
% so indeed the problem is different from:
% 1) random features regression (Song Mei et al 2021) + many more
% 2) learning the best kernel (Sinha-Duchi 2016) 
% we genuinely care about uniform convergence to the kernel approximation as its own end goal, since we want to use the eigendecomposition of that kernel, and the literature doesn't seem to have studied the uniform convergence of kernels beyond shift-invariant kernels which have lipschitz or bounded properties. thus this is a novel result in that line of work as well.

\begin{theorem}[ReLU Kernel Learning Sample Complexity]
Let
\[
\hat{K}_{\sigma} = \frac{1}{N}\sum_{k = 1}^N \sigma(x_k^{\top}W)\sigma(x_k^{\top}W)^{\top}
\]
where $W \in \R^{d \times m}$ satisfies $\|W_i\|_2 \leq R$, $\sigma(a) = \max(0, a)$ for $a \in \R$ is the ReLU activation function and where we draw $N$ samples from the data distribution $\left\{\left(x_k, \sigma(x_k^{\top}W)\right)\right\}_{k = 1}^N$ with $x_k \sim \mathcal{N}\left(0, I_{d \times d}\right)$ i.i.d. for all $k \in [N]$. Now suppose 
\[
N \geq \Omega\left(\frac{R^4\cdot d^2 \cdot m^2}{\eps^2}\cdot \min\left(d\log^2\left(\frac{1}{\delta}\right), \frac{1}{\delta}\right)\right)
\]
Then, with probability at least $1 - \delta$, we have $\|\hat{K}_{\sigma} - K_{\sigma}\|_F \leq \eps$.
\end{theorem}
\begin{proof}
We proceed by analyzing the concentration of the individual kernel values, followed by a union bound over a discretization of the compact space of possible $W$. 
This analysis is very similar to the analysis in \citet{rahimi2007random}; however we must make use of a more involved argument using dependent Hanson-Wright (Lemma~\ref{lem:hanson_wright_dependent}) since our kernel estimate is not a bounded function in the random samples and has more complicated dependencies.

First define the random variable
\[
Z(i, j) := \sigma(x^{\top}W_i)\sigma(x^{\top}W_j)
\]
where $x \sim \mathcal{N}(0, I_{d \times d})$ and $W_i, W_j$ are the $i^{th}$ and $j^{th}$ columns of $W$.
Note that by definition,
\[
\E{x}{Z(i, j)} = K_{\sigma}(i, j) = K_{\sigma}(j, i)
\]
When we want to refer to the $Z(i, j)$ associated with sample $k \in [N]$, we call it $Z_k(i, j)$. For simplicity, we drop the $i, j$ indexing until it is necessary.
Thus, to prove concentration and get a lower bound on the required sample complexity, we want to upper bound
\[
\mathbb{P}\left(\left|\sum_{k = 1}^N Z_k - \E{}{Z_k}\right| > N\cdot t\right)
\]
Now note that $Z_k$ is very similar to a quadratic form -- we want to take advantage of Hanson-Wright style concentration bounds. The main difference is that we have a non-constant matrix in the quadratic form. In particular, we can write $\sum_{k = 1}^N Z_k$ as follows:
\[
\sum_{k = 1}^N Z_k = X^{\top} A(X) X
\]
and thus
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|\sum_{k = 1}^N Z_k - \E{}{Z_k}\right| > N\cdot t\right) 
    \\
    &= \mathbb{P}\left(\left|X^{\top}A(X)X - \E{}{X^{\top}A(X)X}\right| > N\cdot t\right)
\end{split}
\end{align}

where we define
\[
X = \begin{bmatrix} x_1 & \cdots & x_N\end{bmatrix} \in \R^{d\cdot N}
\]
for $x \in R^d$. The variable matrix is defined by
\[
A(X) = \begin{bmatrix} B_{ij}(x_1) &  &  \\
                                                                & \ddots &   \\
                                                                &  & B_{ij}(x_N)
                                                \end{bmatrix} \in \R^{d\cdot N \times d \cdot N}
\]
where the individual blocks on the diagonal are given by
\[
B_{ij}(x) := W_iW_j^{\top} \textbf{1}\left(W_i^{\top}x > 0\right)\textbf{1}\left(W_j^{\top}x > 0\right) \in \R^{d \times d}
\]
We will also refer to $B_{ij} = W_iW_j^{\top}$ when there is no $x$.

Thus we can apply Hanson-Wright if we can reduce to the question to bounding the concentration of each of the $2^N$ possible values of $A(X)$. To enact this strategy, we re-write the bound in terms of different random variables which can be bounded with $N$ different Hanson-Wright concentration bounds, after conditioning on which realization of $A(X)$ shows up. We will be able to do this due to the independence of the $x_1, \cdots, x_N$ as well as the fact that the block diagonals are identically distributed (either $0$ or $B_{ij}$).

In particular, define the random variable
\[
\xi_k := Y_k^{\top}B_{ij}Y_k\cdot I_k - p_{ij}\cdot \E{Y_k}{Y_k^{\top}B_{ij}Y_k}
\]
where we define $I_k$ as the indicator random variable for the event $B_{ij}(x_k) > 0$, and the probability 
\begin{align}
\begin{split}
    p_{ij} &= \mathbb{P}_{x \sim \mathcal{N}(0, I)}\left(B_{ij}(x) \neq 0\right) 
    \\
    &= \mathbb{P}_{x \sim \mathcal{N}(0, I)}\left(W_i^{\top}x \geq 0 \txt{ and } W_j^{\top}x \geq 0\right)
\end{split}
\end{align}

Note that since $I_k$ is i.i.d., $\mathbb{P}\left(I_k\right) = p_{ij}$.
Let the distribution of $Y_k$ be defined conditionally as $x_k | I_k$. 
Now, though $x_k \sim \mathcal{N}(0, I_{d \times d})$ are independent features, dependencies may arise in $Y_k$ as the result of this conditioning. Note that $\xi_k$ are i.i.d. across $k \in [N]$ and also that $\E{}{\xi_k} = 0$.

With these definitions in hand, we can write
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|X^{\top}A(X)X - \E{}{X^{\top}A(X)X}\right| > N\cdot t\right)
    \\
    &= \mathbb{P}\left(\left|\sum_{k = 1}^N x_k^{\top}B_{ij}x_k \cdot I_k - \E{}{x_k^{\top}B_{ij}(x_k)x_k}\right| > N\cdot t\right) 
    \\
    &= \mathbb{P}\left(\left|\sum_{k = 1}^N x_k^{\top}B_{ij}x_k \cdot I_k - p_{ij}\E{}{x_k^{\top}B_{ij}x_k | I_k}\right| > N\cdot t\right) 
    \\
    &= \mathbb{P}\left(\left|\sum_{k = 1}^N Y_k^{\top}B_{ij}Y_k \cdot I_k - p_{ij}\E{Y_k}{Y_k^{\top}B_{ij}Y_k}\right| > N\cdot t\right) 
    \\
    &= \mathbb{P}\left(\left|\sum_{k = 1}^N \xi_k \right| > N\cdot t\right) 
\end{split}
\end{align}
To bound this probability, we will split the bound into two sub-problems: one bounds the concentration of the indicator variable (scaled by some quantities) and the other applies (dependent) Hanson-Wright to bound the concentration of the quadratic forms.
First we need to condition on $Y_k$ to split the problems up: 
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|\sum_{k = 1}^N \xi_k \right| > N\cdot t\right) 
    \\
    &= \EE{Y_1, \cdots, Y_N}{\mathbb{P}\left(\left|\sum_{k = 1}^N \xi_k \mid Y_k \right| > N\cdot t \mid Y_1, \cdots, Y_N\right)}
\end{split}
\end{align}
using the tower property of conditional expectation and the independence of $\xi_k$ to all $Y_j$, $j \neq k$. Now we focus on the probability to bound inside the expectation. The relevant random variables are now the conditioned versions of $\xi_k$. For notational simplicity, we define $\hat{\xi}_k := \xi_k \mid Y_k$.
Now we can write down the following decomposition:
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|\sum_{k = 1}^N \hat{\xi}_k \right| > N\cdot t\right) 
    \\
    &= \mathbb{P}\left(\left|\sum_{k = 1}^N \hat{\xi}_k - \E{I_k}{\hat{\xi}_k} + \sum_{k = 1}^N \E{I_k}{\hat{\xi}_k} \right| > N\cdot t\right)
    \\
    &\leq \mathbb{P}\left(\left|\sum_{k = 1}^N \hat{\xi}_k - \E{I_k}{\hat{\xi}_k}\right| + \left|\sum_{k = 1}^N \E{I_k}{\hat{\xi}_k} \right| > N\cdot t\right)
    \\
    &= \mathbb{P}\left(\left|\sum_{k = 1}^N \E{I_k}{\hat{\xi}_k} \right| > N\cdot \left(t - s\right) \mid J(s)\right)\mathbb{P}\left(J(s)\right)
    \\
    &+ \mathbb{P}\left(\left|\sum_{k = 1}^N \E{I_k}{\hat{\xi}_k} \right| > N\cdot \left(t - s\right) \mid \neg J(s) \right)\mathbb{P}\left(\neg J(s)\right)
    \\
    &\leq \mathbb{P}\left(\left|\sum_{k = 1}^N \E{I_k}{\hat{\xi}_k} \right| > N\cdot \left(t - s\right) \mid \neg J(s) \right) + \mathbb{P}\left(J(s)\right)
\end{split}
\end{align}
where we define the indicator event
\[
J(s) := \textbf{1}\left(s \leq \frac{1}{N}\left|\sum_{k = 1}^N \hat{\xi}_k - \E{I_k}{\hat{\xi}_k}\right| \mid Y_1, \cdots, Y_N\right)
\]
Now, we can take the expectation over the bounds and finally split up the two terms and apply dependent Hanson-Wright to the first term and Bernoulli concentration to the second term. In particular, we have 
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|\sum_{k = 1}^N \xi_k \right| > N\cdot t\right)
    \\
    &\leq \EE{Y_{1:N}}{\mathbb{P}\left(\left|\sum_{k = 1}^N \E{I_k}{\hat{\xi}_k} \right| > N\cdot \left(t - s\right) \mid \neg J(s), Y_{1:N}\right)} 
    \\
    &+ \EE{Y_1, \cdots, Y_N}{\mathbb{P}\left(J(s) \mid Y_1, \cdots, Y_N\right)}
    \\
    &\leq \mathbb{P}\left(\left|\sum_{k = 1}^N Y_k^{\top}B_{ij}Y_k - \E{Y_k}{Y_k^{\top}B_{ij}Y_k} \right| > \frac{N\cdot t}{p_{ij}}\right) 
    \\
    &+ \EE{Y_{1:N}}{\mathbb{P}\left(\frac{1}{N}\left|\sum_{k = 1}^N \hat{\xi}_k - \E{I_k}{\hat{\xi}_k}\right| \geq s \mid Y_{1:N}\right)}
\end{split}
\end{align}
where we used the fact that 
\[
\E{I_k}{\hat{\xi}_k} = p_{ij} \left(Y_k^{\top}B_{ij}Y_k - \E{Y_k}{Y_k^{\top}B_{ij}Y_k}\right)
\]

Now define the mean zero random variable (conditioned on $Y_1, \cdots, Y_k$)
\begin{align}
\begin{split}
\psi_k &:= \hat{\xi}_k - \E{I_k}{\hat{\xi}_k} = Y_k^{\top}B_{ij}Y_k\cdot \left( I_k - p_{ij}\right) 
\\
&= Y_k^{\top}B_{ij}Y_k\cdot \left(I_k - \E{}{I_k}\right)
\end{split}
\end{align}
so after conditioning on $Y_k$, we have a centered $\txt{Bernoulli}(p)$ scaled by a quadratic form in $Y_k$. Thus we can apply Bernoulli concentration via the Hoeffding bound \citep{vershynin2018high}, since the $\psi_k$ are bounded i.i.d. conditioning on the $Y_k$.
We have that the size of the bound interval on $\psi_k$ (conditioning on the $Y_k$) is:
\[
Y_k^{\top}B_{ij}Y_k\cdot \left[\left(1 - p_{ij}\right) - (-p_{ij})\right] = Y_k^{\top}B_{ij}Y_k
\]
Thus, applying Hoeffding, we get
\begin{align}
    &\mathbb{P}\left(\left|\sum_{k = 1}^N \psi_k \right| \geq N\cdot s \mid Y_1, \cdots, Y_N\right)
    \\
    &\leq 2\exp\left(-\frac{2(N\cdot s)^2}{\sum_{k = 1}^N \left(Y_k^{\top}B_{ij}Y_k\right)^2}\right)
\end{align}
Now plugging in the expectation, we get
\begin{align}
\begin{split}
    &\EE{Y_1, \cdots, Y_N}{\mathbb{P}\left(\frac{1}{N}\left|\sum_{k = 1}^N \hat{\xi}_k - \E{I_k}{\hat{\xi}_k}\right| \geq s \mid Y_1, \cdots, Y_N\right)}
    \\
    &\leq 2\EE{Y_1, \cdots, Y_N}{\exp\left(-\frac{2(N\cdot s)^2}{\sum_{k = 1}^N \left(Y_k^{\top}B_{ij}Y_k\right)^2}\right)}
\end{split}
\end{align}

Thus, overall, we have the bound
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|\sum_{k = 1}^N \xi_k \right| > N\cdot t\right)
    \\
    &\leq \mathbb{P}\left(\left|\sum_{k = 1}^N Y_k^{\top}B_{ij}Y_k - \E{Y_k}{Y_k^{\top}B_{ij}Y_k} \right| > N\cdot t\right) 
    \\
    &+ 2\EE{Y_1, \cdots, Y_N}{\exp\left(-\frac{2(N\cdot t)^2}{\sum_{k = 1}^N \left(Y_k^{\top}B_{ij}Y_k\right)^2}\right)}
\end{split}
\end{align}
where we noted that the worst case for the first term is $p_{ij} = 1$ and we defined $s = t$.
We bound the second term in the sum first by replacing $Y_k$ with $X_k$ (this yields an upper bound since $(Y_k^{\top}B_{ij}Y_k)^2$ can only grow larger since it is always positive and because $Y_k$ has more magnitude $0$ terms).
Then, simply note that 
\[
(X_k^{\top}B_{ij}X_k)^2 \leq \|W_i\|_2^2\cdot \|W_j\|_2^2\cdot \|X_k\|_2^4
\]
and we can replace the second term with the upper bound
\[
2\EE{X_1, \cdots, X_N}{\exp\left(-\frac{2(N\cdot t)^2}{R^4\sum_{k = 1}^N \|X_k\|_2^4 }\right)}
\]

Now we condition on the event 
\[
I_2 := \sum_{k = 1}^N \|X_k\|_2^4 < 2 N\cdot d^2
\]
We can therefore bound 
\begin{align}
\begin{split}
    &\EE{X_1, \cdots, X_N}{\exp\left(-\frac{2(N\cdot t)^2}{R^4\sum_{k = 1}^N \|X_k\|_2^4 }\right)}
    \\
    &\leq \EE{X_1, \cdots, X_N}{\exp\left(-\frac{2\cdot N^2 \cdot t^2}{R^4\sum_{k = 1}^N \|X_k\|_2^4 }\right) \mid I_2}\cdot \mathbb{P}(I_2) 
    \\
    &+ \E{X_1, \cdots, X_n}{\exp(0)}\cdot \mathbb{P}(\neg I_2)
    \\
    &\leq \exp\left(-\frac{N \cdot t^2}{R^4\cdot d^2}\right) + \mathbb{P}(\neg I_2)
    \\
    &\leq \exp\left(-\frac{N \cdot t^2}{R^4\cdot d^2}\right) + c_1\cdot \exp\left(-c_2 \cdot d \cdot \sqrt{N} \right)
\end{split}
\end{align}
where in the last step we apply Lemma~\ref{lem:talagrand_bound_fourth_power} and $c_1, c_2 > 0$ are universal constants.


Now we apply dependent Hanson-Wright (Lemma~\ref{lem:hanson_wright_dependent}) to finish the concentration analysis for a single $W_i, W_j$. We first give the Hanson-Wright (sub-exponential) bound for a single block, and then apply Bernstein's inequality \citep{vershynin2018high} for sums of sub-exponential variables to conclude.
First we apply Lemma~\ref{lem:hanson_wright_dependent} to a single block to prove the random variables are sub-exponential:
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|Y_k^{\top}B_{ij}Y_k - \E{Y_k}{Y_k^{\top}B_{ij}Y_k} \right| > t\right)
    \\
    &\leq 2\exp\left(-\min\left\{\frac{t^2}{c_3^2 \cdot \|B_{ij}\|_{\txt{nuclear}}^2}, \frac{t}{c_3\cdot \|B_{ij}\|_{\txt{nuclear}}}\right\}\right)
    \\
    &\leq 2\exp\left(-\min\left\{\frac{t^2}{c_3^2 \cdot R^4}, \frac{t}{c_3\cdot R^2}\right\}\right)
\end{split}
\end{align}
where $c_3$ is a universal constant and where the last line directly follows from the definition of the nuclear and Frobenius norms: namely that $\|M\|_{\txt{nuclear}}^2 \leq \txt{rank}(M)\cdot \|M\|_F^2$ -- here we used the fact that $W_iW_j^{\top}$ is rank $1$ and $\|W_iW_j^{\top}\|_F^2 \leq \|W_i\|_2^2\|W_j\|_2^2 \leq R^4$. Thus the sub-exponential norm for all $k \in [N]$ terms is $\left\|Y_k^{\top}B_{ij}Y_k - \E{Y_k}{Y_k^{\top}B_{ij}Y_k}\right\|_{\psi_1} \leq c_3\cdot R^2$.

Now we apply standard Bernstein concentration for sums of sub-exponential variables (Theorem $2.8.1$ in \citet{vershynin2018high}):
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|\sum_{k = 1}^N Y_k^{\top}B_{ij}Y_k - \E{Y_k}{Y_k^{\top}B_{ij}Y_k} \right| > N\cdot t\right)
    \\
    &\leq 2\exp\left(- c_6\cdot \min\left\{\frac{N^2\cdot t^2}{N\cdot c_3^2 \cdot R^4}, \frac{N \cdot t}{c_3\cdot R^2}\right\}\right)
    \\
    &\leq 2\exp\left(- c_6\cdot N \cdot \min\left\{\frac{t^2}{c_3^2 \cdot R^4}, \frac{t}{c_3\cdot R^2}\right\}\right)
\end{split}
\end{align}


Therefore, putting it all together, we get the bound 
\begin{align}
\begin{split}
    &\mathbb{P}\left(\frac{1}{N}\left|\sum_{k = 1}^N Z_k(i, j) - \E{}{Z_k(i, j)}\right| > t\right)
    \\
    &\leq 2\exp\left(- c_6\cdot N \cdot \min\left\{\frac{t^2}{c_3^2 \cdot R^4}, \frac{t}{c_3\cdot R^2}\right\}\right)
    \\
    & + 2\exp\left(-N\cdot \frac{t^2}{R^4\cdot d^2}\right) + 2c_1\cdot \exp\left(-c_2 \cdot d \cdot \sqrt{N} \right)
\end{split}
\end{align}


Now we need to uniformly bound over all choices of $W_i, W_j$ satisfying $\|W_i\|_2, \|W_j\|_2 \leq R$, so that the above bound holds simultaneously for any pair $W_i, W_j$.
The product of the two $\ell_2$ balls $M := B_{\ell_2}\left(0, R\right) \times B_{\ell_2}\left(0, R\right)$ forms a compact set, so we will proceed by discretizing and arguing that the discretization provides sufficient approximation.
Lemma~\ref{lem:eps_net_union_bound} gives the upper bound on the probability for the failure event that the approximation error of the kernel for any choice of $(W_i, W_j) \in M$ is greater than $\eps$:
\[
\delta = 2 \left((8R)^{2d} \cdot P(\eps/2)\right)^{\frac{1}{d+1}} \cdot \left(\frac{8}{N}\cdot \left(\frac{Rd}{\eps}\right)^2\right)^{\frac{d}{d+1}}
\]
where we previously bounded 
\begin{align}
\begin{split}
    P(\eps/2) &\leq 2\exp\left(- c_6\cdot N \cdot \min\left\{\frac{\eps^2}{4c_3^2 \cdot R^4}, \frac{\eps}{2c_3\cdot R^2}\right\}\right)
    \\
    & + 2\exp\left(-N\cdot \frac{\eps^2}{4R^4\cdot d^2}\right) 
    \\
    & + 2c_1\cdot \exp\left(-c_2 \cdot d \cdot \sqrt{N} \right)
\end{split}
\end{align}
Now we have to choose $N$ appropriately. Consider each of the three terms of the upper bound on $P(\eps/2)$: 
\begin{enumerate}
    \item For the first term, choosing $N = \mathcal{O}\left(\frac{R^4}{\eps^2}\log(6/\delta')\right)$ contributes $\leq \delta'/3$ to $P(\eps/2)$.
    \item For the second term, choosing $N = \mathcal{O}\left(\frac{R^4\cdot d^2}{\eps^2}\log(6/\delta')\right)$ also contributes $\leq \delta'/3$ to $P(\eps/2)$.
    \item For the third term, choosing $N = \mathcal{O}\left(\frac{1}{d^2}\log^2(1/\delta)\right)$ also contributes at most $\delta'/3$ to $P(\eps/2)$. 
\end{enumerate}
Thus, if we choose 
\[
N = \mathcal{O}\left(\frac{R^4}{\eps^2}\log(6/\delta') + \frac{R^4\cdot d^2}{\eps^2}\log(6/\delta') + \frac{1}{d^2}\log^2(1/\delta')\right)
\]
samples, $P(\eps/2) \leq \delta'$. 
Then we can use the result of Lemma~\ref{lem:eps_net_union_bound} to solve for $\delta'$ in terms of the final probability $\delta$:
\begin{align}
\begin{split}
    \delta = 2 \left((8R)^{2d} \cdot \delta'\right)^{\frac{1}{d+1}} \cdot \left(\frac{8}{N}\cdot \left(\frac{Rd}{\eps}\right)^2\right)^{\frac{d}{d+1}}
\end{split}
\end{align}
Note that we can choose $N \geq \frac{R^4\cdot d^2}{\eps^2} \cdot 2048$ (and this is consistent with the previous choice of $N$). This simplifies the equation to
\begin{align}
\begin{split}
    \delta' &= \frac{\delta^{d + 1} \cdot N^d \cdot \eps^{2d}}{2^{10d + 1}\cdot R^{4d} \cdot d^{2d}}
    \\
    &\geq \delta^{d + 1} 2^{d - 1}
    \\
    &\geq \delta^{d + 1}
\end{split}
\end{align}
and thus 
\[
\log(1/\delta') \leq (d + 1)\log(1/\delta)
\]
Plugging this estimate back in to our sample complexity bound gives us the bound in terms of the overall probability of failure $\delta$:
\[
N = \mathcal{O}\left(\frac{R^4\cdot d}{\eps^2}\log(1/\delta) + \frac{R^4\cdot d^3}{\eps^2}\log(1/\delta) + \log^2(1/\delta)\right)
\]

However, we could have also set $N \geq \frac{R^4\cdot d^2}{\eps^2} \cdot 2048 \cdot \frac{1}{\delta}$ -- giving up a logarithmic dependence in $1/\delta$. In this case, we would get $\delta' \geq \delta$, and thus 
\[
N = \mathcal{O}\left(\frac{R^4\cdot d^2}{\eps^2}\frac{1}{\delta}\right)
\]
This bound achieves better dependence on dimension if $\delta > 1/d$. Thus, we can overall summarize the sample complexity as
\[
N = \mathcal{O}\left(\frac{R^4\cdot d^2}{\eps^2}\cdot \min\left(d\log^2\left(\frac{1}{\delta}\right), \frac{1}{\delta}\right)\right)
\]
Finally, if we choose $N$ at least that large, we have that with probability at least $1 - \delta$, $\|K_{\txt{ReLU}} - \hat{K}_{\txt{ReLU}}\|_{\infty} \leq \eps$. We want to convert this into a Frobenius norm bound. Directly bounding, we get \[
\|K_{\txt{ReLU}} - \hat{K}_{\txt{ReLU}}\|_F^2 \leq m^2 \cdot \eps^2
\]
Therefore, choosing $\eps = \eps'/m$ and plugging it in to get the bound in terms of $\eps'$ gives the desired result.
\end{proof}

\begin{lemma}\label{lem:eps_net_union_bound}
Define
\[
P(\eps) := \mathbb{P}\left(\frac{1}{N}\left|\sum_{k = 1}^N Z_k(i, j) - \E{}{Z_k(i, j)}\right| > \eps\right)
\]
where $Z_k(i, j) := \sigma(x_k^{\top}W_i)\sigma(x_k^{\top}W_j)$ is defined for $\sigma$ the ReLU activation, $x_k \sim \mathcal{N}(0, I_{d\times d})$, $\|W_i\|_2, \|W_j\|_2 \leq R$, and where $N$ is the number of samples. 
Then consider the compact set $M := B_{\ell_2}(0, R) \times B_{\ell_2}(0, R)$. The probability that the worst error estimate over points $(W_i, W_j) \in M$ of the kernel value $k_{\txt{ReLU}}(W_i, W_j)$ is worse than $\eps$ is at most
\[
\delta := 2 \left((8R)^{2d} \cdot P(\eps/2)\right)^{\frac{1}{d+1}} \cdot \left(\frac{8}{N}\cdot \left(\frac{Rd}{\eps}\right)^2\right)^{\frac{d}{d+1}}
\]
\end{lemma}
\begin{proof}
To prove this theorem, we adapt the argument of \citet{rahimi2007random}.
We define $k(W_i, W_j) := \E{x}{\sigma(x^{\top}W_i)\sigma(x^{\top}W_j)}$, $s(W_i, W_j) := \frac{1}{N}\sum_{k = 1}^N \sigma(x_k^{\top}W_i)\sigma(x_k^{\top}W_j)$, and $f(W_i, W_j) = s(W_i, W_j) - k(W_i, W_j)$. We want to uniformly bound $f(W_i, W_j) = f\left(\begin{bmatrix} W_i \\ W_j \end{bmatrix}\right)$ over $\begin{bmatrix} W_i \\ W_j \end{bmatrix} \in M$. We will refer to $W = \begin{bmatrix} W_i \\ W_j \end{bmatrix}$. Our strategy will be to first take a $\frac{\eps}{2}$-net of $M$ (which is possible since $M$ is a compact set), then bound the approximation error of a point not in the net to the closest point in the net. To carry out this strategy, we first bound the Lipschitz constant of $f$ (note that $f$ is Lipschitz in $W$, while it is \txt{not} Lipschitz in $x_k$).
First note that the Lipschitz constant is defined as follows:
\[
L_f = \max_{W^* \in M} \left\|\nabla_W f(W^*)\right\|_2
\]
By linearity of expectation we have $\nabla_W k(W) = \E{}{\nabla_W s(W)}$, and therefore we can use the definition of variance to bound
\begin{align}
\begin{split}
    \E{}{L_f^2} &= \E{}{\|\nabla_W f(W^*)\|_2^2}
    \\
    &= \E{}{\|\nabla_W s(W^*) - \nabla_W f(W^*)\|_2^2}
    \\
    &= \E{}{\|\nabla_W s(W^*)\|_2^2} - \E{}{\|\nabla_W f(W^*)\|_2^2}
    \\
    &\leq \E{}{\|\nabla_W s(W^*)\|_2^2}
    \\
    &\leq 2\E{}{\|\nabla_{W_i} s(W^*)\|_2^2}
    \\
    &= 2\EE{x}{\left\|\frac{1}{N}\sum_{k = 1}^N x_k \textbf{1}\left({W_i^*}^{\top}x_k > 0 \right)\sigma\left({W_j^*}^{\top}x_k\right)\right\|_2^2}
    \\
    &\leq \frac{2}{N^2} \sum_{k = 1}^N \EE{x}{\left\|x\cdot \textbf{1}\left({W_i^*}^{\top}x > 0 \right)\sigma\left({W_j^*}^{\top}x\right)\right\|_2^2}
    \\
    &\leq \frac{2}{N}\E{x}{(x{W_j^*}^{\top}x)^{\top}(xW_j^{\top}x)}
    \\
    &= \frac{2}{N}\E{x}{\|x\|_2^2 ({W_j^*}^{\top}x)^2}
    \\
    &\leq \frac{2}{N}\cdot \|W_j^*\|_2^2\cdot \E{x}{\|x\|_2^4}
    \\
    &\leq \frac{2}{N}\cdot R^2 \cdot d^2
\end{split}
\end{align}
where we previously bounded the fourth power of a standard Gaussian $\ell_2$ norm in Lemma~\ref{lem:talagrand_bound_fourth_power}.
For convenience, we define
\[
\sigma^2 := \frac{2}{N}\cdot R^2 \cdot d^2
\]
Then by Markov's inequality, we have 
\[
\mathbb{P}\left(L_f^2 > t\right) \leq \frac{\E{}{L_f^2}}{t} \leq \frac{\sigma^2}{t}
\]
and thus
\[
\mathbb{P}\left(L_f > t\right) \leq \left(\frac{\sigma}{t}\right)^2
\]
We choose $t = \frac{\eps}{2r}$ in order to ensure only an extra $\frac{\eps}{2}$ in approximation error for any point not in the net (here, $r$ is the radius of balls we will choose to determine the size of a cover for the $\frac{\eps}{2}$-net).
Thus we get
\[
\mathbb{P}\left(L_f > \frac{\eps}{2r}\right) \leq \left(\frac{2r\cdot \sigma}{\eps}\right)^2
\]
Then we can apply the union bound over the net of size $T$ to get a uniform bound over the elements of the net:
\[
\mathbb{P}\left(\cup_{s = 1}^T \left\{|f(W_s)| \geq \eps/2\right\}\right) \leq T \cdot P\left(\frac{\eps}{2}\right)
\]
We combine this estimate using another union bound with the bad event that the error for points off the $\frac{\eps}{2}$-net is worse than $\frac{\eps}{2}$ to bound the probability that the error of the worst $W \in M$ is more than $\eps$:
\begin{align}
\begin{split}
    &\mathbb{P}\left(\sup_{W \in M} |f(W)| \geq \eps\right) 
    \\
    &\leq T\cdot P\left(\frac{\eps}{2}\right) + \left(\frac{2r\cdot \sigma}{\eps}\right)^2
    \\
    &\leq \left(\frac{2\txt{diam}(M)}{r}\right)^{2d} \cdot P\left(\frac{\eps}{2}\right) + \left(\frac{2r\cdot \sigma}{\eps}\right)^2
\end{split}
\end{align}
where we used standard upper bounds for the number of $r$-balls which can fit in a compact space with a given diameter in dimension $2d$ (recall $W \in \R^{2d}$ since it is a concatenation of vectors).
Here the bound is of the form
\[
\alpha\cdot r^{-2d} + \beta \cdot r^2
\]
where $\alpha := (8R)^{2d} \cdot P\left(\frac{\eps}{2}\right)$ and $\beta := \frac{8}{N}\left(\frac{Rd}{\eps}\right)^2$.
Here, we have let $r$ be a free parameter. First applying the bound
\[
\txt{diam}\left(M\right) = \sup \left\{\|x - y\|_2: x, y \in M\right\} \leq 2R + 2R = 4R
\]
and then optimizing over $r$ yields 
\[
r^* = \left(\frac{\alpha}{\beta}\right)^{\frac{1}{2d + 2}}
\]
Plugging this optimal choice of $r$ back in yields the bound
\[
2 \alpha^{\frac{1}{d + 1}}\beta^{\frac{d}{d+1}}
\]
Plugging in the values of $\alpha, \beta$ yields the desired result.
\end{proof}

% TODO: add statements of the talagrand theorem (with definitions for orlicz norm etc)
% also add statements of hoeffding bound and bernstein bound from vershynin. 
\begin{lemma}\label{lem:talagrand_bound_fourth_power}
Assume $X_1, \cdots, X_N \in \R^d$ are i.i.d. standard Gaussians drawn from $\mathcal{N}\left(0, I_{d \times d}\right)$.
Then
\[
\mathbb{P}\left(\frac{1}{N}\sum_{k = 1}^N \|X_k\|_2^4 > 2d^2\right) \leq c_1 \cdot \exp\left(-c_2 \cdot d \cdot \sqrt{N} \right)
\]
where $c_1, c_2 > 0$ are universal constants.
\end{lemma}
\begin{proof}
First we need to show that 
\[
\mathbb{P}\left(\left|\|X_k\|_2^4 - \E{}{\|X_k\|_2^4}\right| > t\right) \leq c_1\cdot \exp\left(-c_2\cdot \sqrt{t}\right)
\]
Then, by Theorem $3$ of \citet{talagrand1989isoperimetry} (in particular see the second equation in the proof of Theorem $3$ starting on pg. 1555), we get the concentration bound
\begin{align}
\begin{split}
    &\mathbb{P}\left(\left|\sum_{k = 1}^N \|X_k\|_2^4 - \E{}{\|X_k\|_2^4}\right| > N\cdot t\right) 
    \\
    &\leq c_1\cdot \exp\left(-c_2\cdot \sqrt{N\cdot t}\right)
\end{split}
\end{align}


which completes the desired result.

Thus, we proceed by showing the first statement for the $X_k$.
First we bound the concentration probability of the squared norm of a standard $d$-dimensional Gaussian (see Theorem $3.1.1$ in \citet{vershynin2018high}):
\[
\mathbb{P}\left(\left|\|x\|_2^2 - d\right| > t\cdot d\right) \leq 2\exp\left(-c_5\cdot d\cdot \min(t, t^2)\right)
\]
Then we have
\begin{align}
\begin{split}
    \mathbb{P}\left(\|x\|_2^2 > (1 + t)\cdot d\right) &\leq 2\exp\left(-c_5\cdot d\cdot \min(t, t^2)\right)
    \\
    \mathbb{P}\left(\|x\|_2^4 > (1 + t)^2\cdot d^2\right) &\leq 2\exp\left(-c_5\cdot d\cdot \min(t, t^2)\right)
    \\
    \mathbb{P}\left(\|x\|_2^4 - d^2 > (2t + t^2)\cdot d^2\right) &\leq 2\exp\left(-c_5\cdot d\cdot \min(t, t^2)\right)
\end{split}
\end{align}
Then note that 
\begin{align}
\begin{split}
     &\mathbb{P}\left(\|x\|_2^4 - d^2 > (2t + t^2)\cdot d^2\right)
     \\
     &\geq \mathbb{P}\left(\|x\|_2^4 - d^2 > 3\max\left(t, t^2\right)\cdot d^2\right)
     \\
     &\geq \mathbb{P}\left(\|x\|_2^4 - \E{}{\|x\|_2^4} > 3\max\left(t, t^2\right)\cdot d^2\right)
\end{split}
\end{align}
since by Jensen's inequality, the convexity of the square function, and the fact that $\E{}{\|x\|_2^2} = d$, we have
\[
\E{}{\|x\|_2^4} \leq d^2
\]
Now we have two cases: $t < 1$ and $t \geq 1$. In the first case, $t^2 < t$ and we can plug in our estimates to get the bound
\[
\mathbb{P}\left(\|x\|_2^4 - \E{}{\|x\|_2^4} > 3t\cdot d^2\right) \leq 2\exp\left(-c_5\cdot d\cdot t^2\right)
\]
In the second case, $t^2 \geq t$ and we plug in our bounds to get
\[
\mathbb{P}\left(\|x\|_2^4 - \E{}{\|x\|_2^4} > 3t^2\cdot d^2\right) \leq 2\exp\left(-c_5\cdot d\cdot t\right)
\]
or after variable replacement
\[
\mathbb{P}\left(\|x\|_2^4 - \E{}{\|x\|_2^4} > t\right) \leq 2\exp\left(-(c_5/\sqrt{3})\cdot \sqrt{t}\right)
\]
Thus for any $t > 0$ we have proven the bound
\begin{align}
\begin{split}
    &\mathbb{P}\left(\|x\|_2^4 - \E{}{\|x\|_2^4} > 3t\cdot d^2\right) 
    \\
    &\leq 2\exp\left(-c_5\cdot d\cdot \min\left(t^2, \sqrt{t}\right)\right)
\end{split}
\end{align}

We choose $t > 1$ so that the probability bound isn't increasing in dimension and end up choosing $t = d^2$ for the statement we want, so we end up using the second case version of the bound.
We can apply similar techniques to get the two-sided bound, and finally, we can absorb the constants and the dependence on dimension here into $c_2$ to get the desired result.
\end{proof}

% To get sample complexity bounds that don't depend on minimum eigenvalue / bad eigenvalue gaps, we may need to assume Gaussian W.
% (for general W, we could have small gaps which would blow up eigenvector
% approximation error).
% then, we can make a note of this "average case" style condition
% and connect it to assuming both avg case + structure on non-realizability
% and highlight the existing avg case hardness results which don't apply.
\begin{remark}[Normalized Gaussian Setting] \label{rem:spectral_properties_bounds}
One relevant ``average-case'' setting which is common in practice chooses the $m$ entries of $W$ from a normalized Gaussian $\mathcal{N}(0, \frac{1}{d}I_{d \times d})$ (e.g. He and Glorot initialization \citep{glorot2010understanding, he2015delving}).
In this case, we have $R = \max_{i \in [m]} \|W_i\|_2 = \mathcal{O}\left(1\right)$ with high probability via standard argument (see Theorem $3.1.1$ in \citet{vershynin2018high}) as long as $d \gg \log(m)$ (for union bound purposes), and we can also bound the spectral norm using Mar\v{c}enko-Pastur \citep{marcenko1967distribution} (or more crudely, with another Frobenius norm bound). Mar\v{c}enko-Pastur tells us that we can upper bound $\|W\|_2 \leq \left(1 + \sqrt{d/m}\right)^2$, essentially by a constant.
We can also bound the eigenvalue gaps using Theorem $2.6$ of \citet{nguyen2017random}: with probability at least $1 - \mathcal{O}(m^{-A})$ for $A > 0$, the $r^{th}$ eigenvalue gap of kernel matrix $K_{\sigma}$ satisfies $\lambda_r - \lambda_{r - 1} \geq m^{-B}$. For our case, we can choose to $A$ to be some positive constant and then $B$ can be chosen to be a linear function of $A$. If we factor in this event to the bound (and union bound over this possibility as well), we therefore only experience some additional polynomial blow-up with regards to the dependence on $m$ in Theorem~\ref{thm:efficient_learning}.
\end{remark}

\begin{remark}[Improvements in Polynomial Degrees]\label{rem:improving_degrees}
It is likely that one can reduce the polynomial powers of the $m, R,$ and $\eps$ terms in our bounds in Theorem~\ref{thm:efficient_learning} by more carefully bounding in Lemmas~\ref{lem:perturbation_bound1}, \ref{lem:perturbation_bound2}, and \ref{lem:perturbation_bound3}. Additionally, we can probably remove many factors of $R$ and $m$ by replacing Frobenius norm bounds with spectral norm bounds and working in a setting where the spectral norm is bounded by a constant.
\end{remark}

\begin{remark}[Why Learn the Kernel Matrix Separately from $W$?] \label{rem:why_learn_kernel_separately}
Another approach to running the algorithm is to use the estimated $\hat{W}$ (from gradient descent) in order to calculate an approximate $\hat{K}$ -- in this way, we could potentially avoid the analysis of the concentration of the kernel matrix. However, this approach does not work (at least directly) -- if we try to analyze the resultant kernel matrix values, we can only get \textit{multiplicative} approximations of the error rather than additive (if we try to convert into additive errors, the bounds blow up). This difficulty arises due to having to estimate the cosine of the angles between columns of $W$ -- dealing with estimating the normalization is not easy. Since we are trying to get additive approximations of the error, this approach is not sufficient. % In the perturbation bounds, it doesn't matter since we're not trying to estimate the cosine -- just upper bound it.
\end{remark}

% don't seem to need this.
%\begin{lemma}
%For $B = W_iW_j^{\top}$ with $\|W_i\|_2, \|W_j\|_2 \leq R$
%and $X \sim \mathcal{N}(0, I_{d \times d})$ with
%$Y \sim X \mid \left\{W_i^{\top}X \geq 0 \txt{ and } W_j^{\top}X \geq 0\right\}$,
%\[
%\E{Y}{Y^{\top}BY} \leq R^2 \cdot d
%\]
%\end{lemma}


Since Algorithm~\ref{alg:lowrank_shallow_learning} outputs $\hat{W}\hat{V}\hat{V}^\top$, we only care about the terms $\hat{W}$ and $\hat{V}\hat{V}^\top$. We already have a perturbation bound on $W$ for free. Thus it remains to get a perturbation bound on $VV^\top$. To get this result, we restate a useful variant of the classic Davis-Kahan $\sin(\Theta)$ theorem:

\begin{lemma}[Davis-Kahan $\sin(\Theta)$ Theorem as stated in \citet{yu2015useful}]\label{lem:davis_kahan}
Let $K, \hat{K} \in \R^{m \times m}$ be a real-valued, symmetric with the eigenvalues of $K$ given by $\lambda_1 \geq \cdots \geq \lambda_m$. Since $K$ is real symmetric we can write $K = V \Sigma V^{\top}$. Suppose we take the top $r < m$ eigenvectors $V \in \R^{m \times r}$, which form an orthonormal eigenbasis. Then
\[
\left\|VV^{\top} - \hat{V}\hat{V}^{\top}\right\|_F \leq \frac{2\sqrt{2}\left\|K - \hat{K}\right\|_F}{\lambda_r - \lambda_{r - 1}}
\]
\end{lemma}

% TODO: make note that the eigenvalue gap in the Davis-Kahan is unavoidable in general

% TODO: make note that we can always try to choose ranks so that we avoid this eigenvalue gap (since the actual eigenvectors themselves are not determinable within an eigenspace (though, we don't know W in advance)

% TODO: if W is drawn from a gaussian (or other distributions), work characterizing the eigengap distribution exists and we can bound it with a constant. similarly for maximal eigenvalue (Marchenko Pastur, Wigner Semi-Circle, Tracy-Widom) stuff is relevant - what assumptions should we remark on?

The key lemma tying everything together bounds the suboptimality with respect to $\txt{opt}$ in generalization error of the output of Algorithm~\ref{alg:lowrank_shallow_learning}.
\begin{lemma}[Perturbation Bound I] \label{lem:perturbation_bound1}
Suppose we learn $\hat{W} = W + E$ and $\hat{K}_{\txt{ReLU}} = K_{\txt{ReLU}} + H$ from samples, and $VV^{\top} = \hat{V}\hat{V}^{\top} + F$ where $V$ and $\hat{V}$ are the top-$r$ eigenvectors of $K_{\txt{ReLU}}$ and $\hat{K}_{\txt{ReLU}}$ respectively, and $\lambda_r, \lambda_{r -1}$  are the $r^{th}$ and $(r - 1)^{st}$ eigenvalues of $K_{\txt{ReLU}}$.
Then, we bound the perturbation error
\[
\mathcal{R}(\hat{Y}) - \mathcal{R}(Y^*) \leq 8R^2 \cdot m \cdot \sqrt{\left\|H\right\|_F\frac{\|W\|_2}{\lambda_r - \lambda_{r - 1}} + \|E\|_F}
\]
assuming that we will choose the number of samples to produce $\hat{Y}$ so that $\|F_i\|_2 < 1$.
\end{lemma}
\begin{proof}
First note that since $\|F_i\|_2 < 1$ we have
\begin{align}
\begin{split}
\mathcal{R}(\hat{Y}) - \mathcal{R}(Y^*) \leq 4R^2 \cdot \sum_{i = 1}^m \sqrt{\|F_i\|_2\|W\|_2 + \|E\|_F}
\end{split}
\end{align}
using Lemma~\ref{lem:perturbation_bound2} and Lemma~\ref{lem:perturbation_bound3} and assuming that we will choose the number of samples so that $\|F_i\| < 1$. Now we want to get the dependence on properties of $H$ rather than $F$, via Davis-Kahan. By Davis-Kahan we have
\[
\|F\|_F \leq \frac{2\sqrt{2}\left\|H\right\|_F}{\lambda_r - \lambda_{r - 1}}
\]
Then we can naively bound $\|F_i\|_2 \leq \|F\|_F$, and so we get 
\begin{align}
\begin{split}
\mathcal{R}(\hat{Y}) - \mathcal{R}(Y^*) &\leq 4R^2 \cdot m \cdot \sqrt{\|F\|_F\|W\|_2 + \|E\|_F}
\\
&\leq 8R^2 \cdot m \cdot \sqrt{\left\|H\right\|_F\frac{\|W\|_2}{\lambda_r - \lambda_{r - 1}} + \|E\|_F}
\end{split}
\end{align}
\end{proof}


First we relate the generalization gap  to the cosine of the angles between the optimum $Y^*$ and the sample optimum $\hat{Y}$:

\begin{lemma}[Perturbation Bound II]\label{lem:perturbation_bound2}
Let $R = \max_{i \in [m]} \|W_i\|_2$.
For the objective defined in Problem~\ref{prob:learning_prob_statement}, we have that for $\hat{Y}$ which minimize the population version of the objective with $\hat{W}, \hat{K}$ as the ground truth (e.g. the output of Algorithm~\ref{alg:mixnmatch} on the sample versions of $\hat{W}$ and $\hat{K}$) that
\[
\mathcal{R}(\hat{Y}) - \mathcal{R}(Y^*) \leq \sqrt{2}\cdot R^2 \cdot \sum_{i = 1}^m \sqrt{1 - \cos\left(\Theta(Y_i^*, \hat{Y}_i)\right)}
\]
\end{lemma}
\begin{proof}
Using the representation from Theorem~\ref{thm:relu_svd}, we write
\begin{align}
\begin{split}
    \mathcal{R}(\hat{Y}) - \mathcal{R}(Y^*) &= \frac{1}{2}\sum_{i = 1}^m \left(h(\rho_i^*) - h(\hat{\rho}_i)\right) \|W_i\|_2^2
    \\
    &\leq \frac{R^2}{2} \sum_{i = 1}^m (\sqrt{h}(\rho_i^*) + \sqrt{h}(\hat{\rho}_i))\cdot(\sqrt{h}(\rho_i^*) - \sqrt{h}(\hat{\rho}_i))
    \\
    &\leq R^2 \sum_{i = 1}^m (\sqrt{h}(\rho_i^*) - \sqrt{h}(\hat{\rho}_i))
    \\
    &\leq R^2 \sum_{i = 1}^m \frac{1}{2}(\rho_i^* - \hat{\rho}_i) + \frac{1}{\pi}\sum_{\ell = 1}^{\infty} c_{\ell}^2 ({\rho_i^*}^{2\ell} - {\hat{\rho_i}}^{2\ell})
    \\
    &\leq R^2 \sum_{i = 1}^m \left(\frac{1}{2} + \frac{1}{2} - \frac{1}{\pi}\right)(\rho_i^* - \hat{\rho}_i) 
    \\
    &\leq R^2 \left\|\rho^* - \hat{\rho}\right\|_1
\end{split}
\end{align}
since $\sqrt{h} \in [1/\pi, 1]$ for $\rho \in [0, 1]$.
Now we write 
\begin{align}
\begin{split}
    \theta_i^* &:= \txt{arccos}\left(\frac{{Y_i^*}^{\top}W_i}{\|Y_i^*\|_2\|W_i\|_2}\right)
    \\
    \hat{\theta}_i &:= \txt{arccos}\left(\frac{{\hat{Y}_i}^{\top}W_i}{\|\hat{Y}_i\|_2\|W_i\|_2}\right)
\end{split}
\end{align}
and note that we wish to bound the terms $\rho_i^* - \hat{\rho}_i = \cos(\theta_i^*) - \cos(\hat{\theta}_i)$. We have
\begin{align}
\begin{split}
    \cos(\theta_i^*) - \cos(\hat{\theta}_i) &= \left(\frac{{Y_i^*}}{\|Y_i^*\|_2} -\frac{{\hat{Y}_i}}{\|\hat{Y}_i\|_2}\right)^{\top}\left(\frac{W_i}{\|W_i\|_2}\right)
    \\
    &\leq \left\|\frac{{Y_i^*}}{\|Y_i^*\|_2} -\frac{{\hat{Y}_i}}{\|\hat{Y}_i\|_2}\right\|_2
    \\
    &\leq \sqrt{2\left(1 - \cos\left(\Theta(Y_i^*, \hat{Y}_i)\right)\right)}
\end{split}
\end{align}
where we applied Cauchy-Schwarz and the definition of cosine. Plugging in this upper bound yields the theorem.
\end{proof}


\begin{lemma}[Perturbation Bound III] \label{lem:perturbation_bound3}
Suppose we learn $\hat{W} = W + E$ and $\hat{K}_{\txt{ReLU}} = K_{\txt{ReLU}} + H$ from samples, and $VV^{\top} = \hat{V}\hat{V}^{\top} + F$ where $V$ and $\hat{V}$ are the eigenvectors of $K_{\txt{ReLU}}$ and $\hat{K}_{\txt{ReLU}}$ respectively.
Then, we bound the perturbation error
\[
1 - \cos\left(\Theta(Y_i^*, \hat{Y}_i)\right) \leq (1 + \pi + \|F_i\|_2)\left(\|F_i\|_2\|W\|_2 + \|E\|_F\right)
\]
in terms of properties of $E, F, W, $ and $K_{\txt{ReLU}}$, where $\hat{Y}$ is the optimum reconstruction for $\hat{W}, \hat{K}_{\txt{ReLU}}$, noting that as $\|E\|_F, \|F_i\|_2 \to 0$, the upper bound tends to $0$.
\end{lemma}
\begin{proof}
Define $K_{\txt{ReLU}} = V\Sigma V^{\top}$ and $\hat{K}_{\txt{ReLU}} = \hat{V}\hat{\Sigma}\hat{V}^{\top}$ since the kernel matrix is real symmetric. Let $\hat{V}\hat{V}^{\top} = VV^{\top} + F$. We will use $V_i$ to denote the $i^{th}$ column of $V^{\top}$.
First note we have by Algorithm~\ref{alg:mixnmatch}
\begin{align}
\begin{split}
    Y^* &= WVV^{\top}
    \\
    \hat{Y} &= \hat{W}\hat{V}\hat{V}^{\top}
\end{split}
\end{align}
Then we need to lower bound $\cos\left(\Theta(Y_i^*, \hat{Y}_i)\right)$. 
\begin{align}
\begin{split}
    \cos\left(\Theta(Y_i^*, \hat{Y}_i)\right) &= \frac{\left(WVV_i\right)^{\top}(W + E)\hat{V}\hat{V}_i}{\|WVV_i\|_2\cdot\|(W + E)\hat{V}\hat{V}_i\|_2}
    \\
    &= \frac{\langle W(VV_i + F_i), WVV_i \rangle}{\|WVV_i\|_2\cdot\|(W + E)(VV_i + F_i)\|_2} 
    \\ 
    &+ \frac{\langle E(VV_i + F_i), WVV_i \rangle}{\|WVV_i\|_2\cdot\|(W + E)(VV_i + F_i)\|_2}
\end{split}
\end{align}
We lower bound the two terms separately. First:
\begin{align}
\begin{split}
    &\frac{\langle W(VV_i + F_i), WVV_i \rangle}{\|WVV_i\|_2\cdot\|(W + E)(VV_i + F_i)\|_2} 
    \\
    &\geq \frac{\|WVV_i\|_2}{\|WVV_i\|_2 + \|WF_i\|_2 + \|EVV_i\|_2 + \|EF_i\|_2}
    \\
    &+ \frac{\langle WF_i, WVV_i\rangle}{\|WVV_i\|_2\cdot\|(W + E)(VV_i + F_i)\|_2}
    \\
    &\geq s_i - \|F_i\|_2\frac{\|W\|_2}{\cdot\|(W + E)(VV_i + F_i)\|_2}
    \\
    &\geq s_i - \|F_i\|_2\cdot \frac{\|W\|_2}{\|\hat{Y}_i\|_2} \geq s_i - \|F_i\|_2\cdot \pi\|W\|_2
\end{split}
\end{align}
where we applied Cauchy-Schwarz and since we know that $\|\hat{Y}_i\|_2 = \sqrt{h}(\hat{\rho}_i) \geq 1/\pi$ from Theorem~\ref{thm:relu_svd}. Here we define
\[
s_i = \frac{\|WVV_i\|_2}{\|WVV_i\|_2 + \|W\|_2\|F_i\|_2 + \|E\|_F + \|E\|_F\|F_i\|_2}
\]
Note $s_i \in [0, 1]$.
Now we handle the second term:
\begin{align}
\begin{split}
    &\frac{\langle E(VV_i + F_i), WVV_i \rangle}{\|WVV_i\|_2\cdot\|(W + E)(VV_i + F_i)\|_2}
    \\
    &\geq - \|E\|_F\frac{\|\hat{V}\hat{V}_i\|_2}{\cdot\|\hat{Y}_i\|_2}
    \\
    &= -\pi\|E\|_F
\end{split}
\end{align}
Putting it all together, we get 
\[
1 - \cos\left(\Theta(Y_i^*, \hat{Y}_i)\right) \leq 1 - s_i + \pi\left(\|F_i\|_2\|W\|_2 + \|E\|_F\right)
\]
Finally, we can bound $1 - s_i$:
\begin{align}
\begin{split}
    1 - s_i &= \frac{\|W\|_2\|F_i\|_2 + \|E\|_F + \|E\|_F\|F_i\|_2}{\|WVV_i\|_2 + \|W\|_2\|F_i\|_2 + \|E\|_F + \|E\|_F\|F_i\|_2}
    \\
    &\leq \|W\|_2\|F_i\|_2 + \|E\|_F + \|E\|_F\|F_i\|_2
\end{split}
\end{align}
giving the result.
\end{proof}

==> tables_old_copy.tex <==
\begin{figure}
\centering
\begin{tabular}{|c|c|c|}
\hline
 Rank Scale & Method & Avg. Top-$1$ Acc. \\ \hline
 \multirow{4}{*}{0.05} & Baseline &  $58.61 \pm 0.45$ \\ \cline{2-3}
 & Spectral &  $58.84 \pm 0.38$ \\ \cline{2-3}
 & \algnameshort & $59.00 \pm 0.18$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{59.63 \pm 0.37}$  \\ \hline
 \multirow{4}{*}{0.10} & Baseline &  $68.89 \pm 0.07$ \\ \cline{2-3}
 & Spectral &  $68.83 \pm 0.16$ \\ \cline{2-3}
 & \algnameshort & $68.52 \pm 0.04$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{69.09 \pm 0.16}$  \\ \hline
 \multirow{4}{*}{0.15} & Baseline &  $71.67 \pm 0.19$ \\ \cline{2-3}
 & Spectral &  $71.55 \pm 0.20$ \\ \cline{2-3}
 & \algnameshort & $71.25 \pm 0.12$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{71.74 \pm 0.02}$  \\ \hline
  \multirow{4}{*}{0.20} & Baseline &  $72.16 \pm 0.27$ \\ \cline{2-3}
 & Spectral &  $72.45 \pm 0.17$ \\ \cline{2-3}
 & \algnameshort & $72.32 \pm 0.18$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{72.72 \pm 0.03}$  \\ \hline
 1.0 & Full-Rank & TODO \\ \hline
\end{tabular}
\caption{EfficientNet-b7 (Weight Decay)}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|c|c|c|}
\hline
 Rank Scale & Method & Avg. Top-$1$ Acc. \\ \hline
 \multirow{4}{*}{0.05} & Baseline &  $37.34 \pm 0.29$ \\ \cline{2-3}
 & \textbf{Spectral} &  $\mathbf{38.3 \pm 0.09}$ \\ \cline{2-3}
 & \textbf{\algnameshort} & $\mathbf{38.22 \pm 0.28}$  \\ \cline{2-3}
 & WS-\algnameshort & $38.04 \pm 0.03$  \\ \hline
 \multirow{4}{*}{0.10} & \textbf{Baseline} &  $\mathbf{57.06 \pm 0.24}$ \\ \cline{2-3}
 & Spectral &  $56.66 \pm 0.35$ \\ \cline{2-3}
 & \textbf{\algnameshort} & $\mathbf{56.96 \pm 0.19}$  \\ \cline{2-3}
 & WS-\algnameshort & $56.76 \pm 0.11$  \\ \hline
 \multirow{4}{*}{0.15} & Baseline &  $62.56 \pm 0.07$ \\ \cline{2-3}
 & Spectral &  $63.02 \pm 0.07$ \\ \cline{2-3}
 & \algnameshort & $62.86 \pm 0.12$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{63.55 \pm 0.16}$  \\ \hline
  \multirow{4}{*}{0.20} & Baseline &  $66.05 \pm 0.23$ \\ \cline{2-3}
 & Spectral &  $65.96 \pm 0.29$ \\ \cline{2-3}
 & \algnameshort & $65.93 \pm 0.06$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{66.32 \pm 0.02}$  \\ \hline
 1.0 & Full-Rank & TODO \\ \hline
\end{tabular}
\caption{EfficientNet-b3 (Weight Decay)}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|c|c|c|}
\hline
 Rank Scale & Method & Avg. Top-$1$ Acc.   \\ \hline
 \multirow{4}{*}{0.05} & Baseline &  $31.22 \pm 0.62$ \\ \cline{2-3}
 & Spectral &  $30.96 \pm 0.32$ \\ \cline{2-3}
 & \textbf{\algnameshort} & $\mathbf{32.39 \pm 0.26}$  \\ \cline{2-3}
 & WS-\algnameshort & $30.8 \pm 0.19$  \\ \hline
 \multirow{4}{*}{0.10} & \textbf{Baseline} &  $\mathbf{48.24 \pm 0.13}$ \\ \cline{2-3}
 & Spectral &  $47.79 \pm 0.17$ \\ \cline{2-3}
 & \algnameshort & $47.42 \pm 0.30$  \\ \cline{2-3}
 & WS-\algnameshort & $47.84 \pm 0.24$  \\ \hline
 \multirow{4}{*}{0.15} & Baseline &  $54.99 \pm 0.05$ \\ \cline{2-3}
 & Spectral &  $54.97 \pm 0.10$ \\ \cline{2-3}
 & \algnameshort & $54.85 \pm 0.09$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{55.19 \pm 0.10}$  \\ \hline
  \multirow{4}{*}{0.20} & \textbf{Baseline} &  $\mathbf{59.78 \pm 0.17}$ \\ \cline{2-3}
 & Spectral &  $59.42 \pm 0.32$ \\ \cline{2-3}
 & \algnameshort & $59.20 \pm 0.11$  \\ \cline{2-3}
 & WS-\algnameshort & $59.38 \pm 0.18$  \\ \hline
 1.0 & Full-Rank & TODO \\ \hline
\end{tabular}
\caption{EfficientNet-b0 (Weight Decay)}
\end{figure}


% do the same table as above for ResNet-50


\begin{figure}
\centering
\begin{tabular}{|c|c|c|}
\hline
 Rank Scale & Method & Avg. Top-$1$ Acc.   \\ \hline
 \multirow{4}{*}{0.05} & Baseline &  $56.92 \pm 0.14$ \\ \cline{2-3}
 & Spectral &  $56.28 \pm 0.39$ \\ \cline{2-3}
 & \algnameshort & $56.55 \pm 0.04$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{57.37 \pm 0.08}$  \\ \hline
 \multirow{4}{*}{0.10} & Baseline &  $64.09 \pm 0.12$ \\ \cline{2-3}
 & Spectral &  $64.06 \pm 0.19$ \\ \cline{2-3}
 & \algnameshort & $64.02 \pm 0.17$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{64.74 \pm 0.04}$  \\ \hline
 \multirow{4}{*}{0.15} & Baseline &  $67.58 \pm 0.15$ \\ \cline{2-3}
 & Spectral &  $66.95 \pm 0.16$ \\ \cline{2-3}
 & \algnameshort & $67.24 \pm 0.26$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{67.74 \pm 0.03}$  \\ \hline
  \multirow{4}{*}{0.20} & \textbf{Baseline} &  $\mathbf{69.04 \pm 0.33}$ \\ \cline{2-3}
 & Spectral &  $68.59 \pm 0.19$ \\ \cline{2-3}
 & \algnameshort & $68.93 \pm 0.20$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{69.37 \pm 0.07}$  \\ \hline
 1.0 & Full-Rank & $78.1$ \\ \hline
\end{tabular}
\caption{ResNet-50 (Weight Decay)}
\end{figure}


\begin{figure}
\centering
\begin{tabular}{|c|c|c|}
\hline
 Rank Scale & Method & Avg. Top-$1$ Acc.   \\ \hline
 \multirow{4}{*}{0.05} & Baseline &  $57.73 \pm 0.23$ \\ \cline{2-3}
 & Spectral &  $57.42 \pm 0.38$ \\ \cline{2-3}
 & \algnameshort & $57.61\pm 0.15$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{58.22 \pm 0.31}$  \\ \hline
 \multirow{4}{*}{0.10} & Baseline &  $65.61 \pm 0.09$ \\ \cline{2-3}
 & Spectral &  $65.69 \pm 0.12$ \\ \cline{2-3}
 & \algnameshort & $65.55 \pm 0.05$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{65.93 \pm 0.05}$  \\ \hline
 \multirow{4}{*}{0.15} & \textbf{Baseline} &  $\mathbf{68.15 \pm 0.20}$ \\ \cline{2-3}
 & \textbf{Spectral} &  $\mathbf{68.21 \pm 0.08}$ \\ \cline{2-3}
 & \algnameshort & $67.13 \pm 0.51$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{67.83 \pm 0.42}$  \\ \hline
  \multirow{4}{*}{0.20} & Baseline &  $69.22 \pm 0.05$ \\ \cline{2-3}
 & Spectral &  $69.04 \pm 0.14$ \\ \cline{2-3}
 & \algnameshort & $68.87 \pm 0.10$  \\ \cline{2-3}
 & \textbf{WS-\algnameshort} & $\mathbf{69.47 \pm 0.09}$  \\ \hline
 1.0 & Full-Rank & $78.1$ \\ \hline
\end{tabular}
\caption{ResNet-50 (Frobenius Decay)}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|l|l|l|}
\hline
 Rank Scale & Top-$1$ Accuracy for WS-\algnameshort  \\  \hline
 $0.05$ & $59.63 \pm 0.37$  (best by $0.63$) \\ \hline
 $0.1$ & $69.09 \pm 0.16$ (best by $0.20$) \\ \hline
 $0.15$ & $71.74 \pm 0.02$ (best by $0.07$) \\ \hline
 $0.2$ & $72.72 \pm 0.03$ (best by $0.27$) \\ \hline
 Full-Rank & $78.1$  \\ \hline
\end{tabular}
\caption{Comparison of WS-\algnameshort Across Rank Scales for EfficientNet-b7. We show by how many percent points the best performing method, WS-\algnameshort, beats the other methods, for the Weight Decay regularization.}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|l|l|l|}
\hline
 Rank Scale & Top-$1$ Accuracy for \algnameshort  \\  \hline
 $0.05$ & $38.22 \pm 0.28$  (overlaps w/best) \\ \hline
 $0.1$ & $56.96 \pm 0.19$ (overlaps w/best) \\ \hline
 $0.15$ & $63.55 \pm 0.16$ (best by $0.53$) \\ \hline
 $0.2$ & $66.32 \pm 0.02$ (best by $0.27$) \\ \hline
 Full-Rank & $78.1$  \\ \hline
\end{tabular}
\caption{Comparison of \algnameshort Across Rank Scales for EfficientNet-b3. We show by how many percent points the best performing method, \algnameshort, beats the other methods, for the Weight Decay regularization.}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|l|l|l|}
\hline
 Rank Scale & Top-$1$ Accuracy for \algnameshort or WS-\algnameshort  \\  \hline
 $0.05$ & $32.39 \pm 0.26$  (best by $1.17$) \\ \hline
 $0.1$ & $47.84 \pm 0.24$ (suboptimal) \\ \hline
 $0.15$ & $55.19 \pm 0.10$ (best by $0.20$) \\ \hline
 $0.2$ & $59.38 \pm 0.18$ (suboptimal) \\ \hline
 Full-Rank & $78.1$  \\ \hline
\end{tabular}
\caption{Comparison of \algnameshort and WS-\algnameshort Across Rank Scales for EfficientNet-b0. We show by how many percent points WS-\algnameshort compares against the other methods, for the Weight Decay regularization.}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|l|l|l|}
\hline
 Rank Scale & Top-$1$ Accuracy for WS-\algnameshort  \\  \hline
 $0.05$ & $57.37 \pm 0.08$  (best by $0.45$) \\ \hline
 $0.1$ & $64.74 \pm 0.04$ (best by $0.65$) \\ \hline
 $0.15$ & $67.74 \pm 0.03$ (best by $0.16$) \\ \hline
 $0.2$ & $69.37 \pm 0.07$ (best by $0.33$) \\ \hline
 $0.25$ & $70.37 \pm 0.06$ (best by $0.25$) \\ \hline
 Full-Rank & $78.1$  \\ \hline
\end{tabular}
\caption{Comparison of WS-\algnameshort Across Rank Scales for EfficientNet-b7. We show by how many percent points the best performing method, WS-\algnameshort, beats the other methods, for the Weight Decay regularization.}
\end{figure}


\begin{figure}
\centering
\begin{tabular}{|l|l|l|}
\hline
 Rank Scale & Top-$1$ Accuracy for WS-\algnameshort  \\  \hline
 $0.05$ & $57.37 \pm 0.08$  (best by $0.45$) \\ \hline
 $0.1$ & $64.74 \pm 0.04$ (best by $0.65$) \\ \hline
 $0.15$ & $67.74 \pm 0.03$ (best by $0.16$) \\ \hline
 $0.2$ & $69.37 \pm 0.07$ (best by $0.33$) \\ \hline
 $0.25$ & $70.37 \pm 0.06$ (best by $0.25$) \\ \hline
 Full-Rank & $78.1$  \\ \hline
\end{tabular}
\caption{Comparison of WS-\algnameshort Across Rank Scales for ResNet-50. We show by how many percent points the best performing method, WS-\algnameshort, beats the other methods, for the Weight Decay regularization.}
\end{figure}

\begin{figure}
\begin{tabular}{|l|l|l|}
\hline
 Rank Scale & Top-$1$ Accuracy for WS-\algnameshort \\  \hline
 $0.05$ & $58.22 \pm 0.31$ (best by $0.49$) \\ \hline
 $0.1$ & $65.93 \pm 0.05$ (best by $0.24$) \\ \hline
 $0.15$ & $67.83 \pm 0.42$ (sub-optimal) \\ \hline
 $0.2$ & $69.47 \pm 0.09$ (best by $0.25$) \\ \hline
 $0.25$ & $70.16 \pm 0.09$ (best by $0.19$) \\ \hline
 Full-Rank & $78.1$  \\ \hline
\end{tabular}
\caption{Comparison of WS-\algnameshort Across Rank Scales for ResNet-50. We show by how many percent points the best performing method, WS-\algnameshort, beats the other methods, for the Frobenius Decay regularization.}
\end{figure}

